IGASA: Integrated Geometry-Aware and Skip-Attention Modules for Enhanced Point Cloud Registration

Point cloud registration (PCR) is a fundamental task in 3D vision and provides essential support for applications such as autonomous driving, robotics, and environmental modeling. Despite its widespread use, existing methods often fail when facing real-world challenges like heavy noise, significant occlusions, and large-scale transformations. These limitations frequently result in compromised registration accuracy and insufficient robustness in complex environments. In this paper, we propose IGASA as a novel registration framework constructed upon a Hierarchical Pyramid Architecture (HPA) designed for robust multi-scale feature extraction and fusion. The framework integrates two pivotal components consisting of the Hierarchical Cross-Layer Attention (HCLA) module and the Iterative Geometry-Aware Refinement (IGAR) module. The HCLA module utilizes skip attention mechanisms to align multi-resolution features and enhance local geometric consistency. Simultaneously, the IGAR module is designed for the fine matching phase by leveraging reliable correspondences established during coarse matching. This synergistic integration within the architecture allows IGASA to adapt effectively to diverse point cloud structures and intricate transformations. We evaluate the performance of IGASA on four widely recognized benchmark datasets including 3D(Lo)Match, KITTI, and nuScenes. Our extensive experiments consistently demonstrate that IGASA significantly surpasses state-of-the-art methods and achieves notable improvements in registration accuracy. This work provides a robust foundation for advancing point cloud registration techniques while offering valuable insights for practical 3D vision applications. The code for IGASA is available in \href{https://github.com/DongXu-Zhang/IGASA}{https://github.com/DongXu-Zhang/IGASA}.

==> sec/0_abstract.tex <==
\begin{abstract}

% Point cloud registration is a cornerstone task in 3D vision, underpins numerous applications, including autonomous driving, robotics, and environmental modeling. Despite its importance, existing methods often falter when confronted with real-world challenges such as noise, occlusions, and large-scale transformations, leading to compromised accuracy and robustness.
% In this paper, we introduce IGASA, a novel registration framework built upon a Hierarchical Pyramid Architecture (HPA) designed for robust multi-scale feature extraction and fusion. IGASA integrates two pivotal components: the Hierarchical Cross-Layer Attention (HCLA) module and the Iterative Geometry-Aware Refinement (IGAR) module. Specifically, the HCLA module employs skip attention mechanisms to seamlessly align multi-resolution features, thereby enhancing local geometric consistency. Concurrently, the IGAR module is meticulously crafted for the fine matching phase, leveraging reliable correspondences established during coarse matching. This synergistic integration within the HPA enables IGASA to adapt effectively to diverse point cloud structures and intricate transformations.
% We evaluate IGASA on four widely recognized benchmark datasets: 3D(Lo)Match, KITTI, and nuScenes. Our extensive experiments consistently demonstrate that IGASA significantly surpasses state-of-the-art methods, achieving notable improvements in registration accuracy. This work not only provides a robust foundation for advancing point cloud registration techniques but also offers valuable insights for practical 3D vision applications. The code for IGASA is available in \href{https://github.com/DongXu-Zhang/IGASA}{https://github.com/DongXu-Zhang/IGASA}.


Point cloud registration (PCR) is a fundamental task in 3D vision and provides essential support for applications such as autonomous driving, robotics, and environmental modeling. Despite its widespread use, existing methods often fail when facing real-world challenges like heavy noise, significant occlusions, and large-scale transformations. These limitations frequently result in compromised registration accuracy and insufficient robustness in complex environments.
\rev{In this paper, we propose IGASA as a novel registration framework constructed upon a Hierarchical Pyramid Architecture (HPA) designed for robust multi-scale feature extraction and fusion. The framework integrates two pivotal components consisting of the Hierarchical Cross-Layer Attention (HCLA) module and the Iterative Geometry-Aware Refinement (IGAR) module. The HCLA module utilizes skip attention mechanisms to align multi-resolution features and enhance local geometric consistency. Simultaneously, the IGAR module is designed for the fine matching phase by leveraging reliable correspondences established during coarse matching. This synergistic integration within the architecture allows IGASA to adapt effectively to diverse point cloud structures and intricate transformations.}
We evaluate the performance of IGASA on four widely recognized benchmark datasets including 3D(Lo)Match, KITTI, and nuScenes. Our extensive experiments consistently demonstrate that IGASA significantly surpasses state-of-the-art methods and achieves notable improvements in registration accuracy. This work provides a robust foundation for advancing point cloud registration techniques while offering valuable insights for practical 3D vision applications. The code for IGASA is available in \href{https://github.com/DongXu-Zhang/IGASA}{https://github.com/DongXu-Zhang/IGASA}.

\end{abstract}
\begin{IEEEkeywords}
3-D vision, attention mechanism, point cloud matching, point cloud registration.
\end{IEEEkeywords}

==> sec/1_intro.tex <==
\section{Introduction}

Point Cloud Registration (PCR) is a critical task in 3D computer vision, aimed at aligning point clouds captured from different viewpoints or at different time instances to achieve data fusion and complementary information integration~\cite{zhang2024comprehensive}. This process plays a critical role in various applications, such as autonomous driving~\cite{wang2022residual,huang2024kdd}, robot navigation~\cite{wang2022efficient,wang2021deep}, and environmental modeling, where accurate alignment is essential for high-precision perception and decision-making. However, the inherent challenges associated with point cloud data-such as noise, occlusion, non-uniform sampling, and complex transformations ($e.g.,$ large rotations and scaling), significantly hinder both the accuracy and efficiency of registration methods~\cite{bai2021pointdsc}~\cite{qin2022geometric,she2024pointdifformer},~\cite{yew2022regtr}. These issues complicate the registration process, leading to potential inaccuracies and inefficiencies.

\IEEEpubidadjcol

Traditional registration techniques, notably the Iterative Closest Point (ICP) algorithm and its variants~\cite{jost2002fast,vizzo2023kiss},~\cite{sharp2002icp} rely on minimizing point-to-point distances. Although ICP is widely used, it exhibits significant sensitivity to the initialization of parameters. This sensitivity can lead to convergence on local minima, especially when the initial guess is poor or when the data is heavily corrupted by noise and occlusion. Variants of ICP attempt to mitigate these issues, but they still fall short under severe conditions~\cite{yang2015go}. 


\rev{Rigid point cloud registration aims to determine the optimal rotation and translation to align two overlapping point clouds. Correspondence based methods\cite{qin2022geometric,xu2024igreg} generally tackle this task by establishing reliable point matches through a multi stage pipeline. The process typically begins with detecting keypoints and encoding their local geometric properties into feature descriptors. These descriptors are subsequently matched via nearest neighbor search to generate initial correspondences. The final transformation is then computed using robust estimators, such as RANSAC\cite{fischler1981random}, to ensure accurate alignment despite potential outliers.}

% Rigid point cloud registration seeks the optimal rotation and translation to align two point clouds. Correspondence based~\cite{qin2022geometric,xie2024hecpg,xu2024igreg} techniques in this realm typically involve a series of steps: first, keypoints are identified using various detectors; next, feature descriptors are extracted to characterize local geometries; then, these features are matched using nearest neighbor search strategies; and finally, transformation estimation is performed using robust methods like RANSAC~\cite{fischler1981random}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{fig1.pdf}
    \caption{The Inlier Ratio (IR) is plotted on the x-axis for 3DMatch and on the y-axis for 3DLoMatch. IGASA stands out by consistently achieving the highest IR.}
    \label{figurelabel}
    \vspace{-5mm}
\end{figure}

% Recently, deep learning methods have emerged as a promising alternative, offering end-to-end solutions that learn feature representations directly from the raw point cloud data ~\cite{huang2021predator,wang2022you},~\cite{yu2021cofinet}. 

\rev{Recently, deep learning methods have emerged as a promising alternative, demonstrating powerful capabilities in adaptive feature extraction~\cite{zhang2024adaptive}, and offering end-to-end solutions that learn feature representations directly from raw point cloud data~\cite{huang2021predator,yu2021cofinet}.}
Convolutional Neural Networks (CNNs) have been successfully applied for local feature extraction~\cite{9010002}. However, CNNs are constrained by fixed receptive fields that limit their ability to capture long-range dependencies. In contrast, transformer-based architectures ~\cite{qin2022geometric,yang2022one,yu2023rotation},\cite{chen2023sira,huang2017coarse} have demonstrated efficacy in capturing global context, a capability that is particularly advantageous for modeling the overall shape and structure of point clouds. Moreover, advances in deformable image registration have illustrated the benefits of integrating hierarchical and attention mechanisms, where short range self-attentions are complemented by cross-attention strategies to capture broader contextual information~\cite{xie2023cross,xu2024igreg},~\cite{ren2022corri2p,an2024ol}. These methods underscore the necessity of incorporating multi-scale representations to accurately model deformation fields and, by extension, improve point cloud registration.

Motivated by these developments, we propose IGASA, builds on these advancements by integrating a multi-scale hierarchical pyramid architecture (HPA) with two key modules: the Hierarchical Cross-Layer Attention (HCLA) module and the Iterative Geometry-Aware Refinement (IGAR) module. 

The HPA is designed to extract and fuse features at multiple scales, ensuring that both global context and fine local details are effectively captured. Within this framework, the HCLA module employs a skip attention mechanism to seamlessly align multi-resolution features, thereby enhancing local geometric consistency across scales. In practice, the skip attention mechanism weights the contributions from various layers based on their relevance to the registration task, thereby reducing the negative impact of noise and occlusion. 

Complementarily, the IGAR module is specifically designed for the fine matching phase. In each iteration, \rev{the module utilizes geometric cues such as spatial distribution and geometric alignment consistency to assess and enhance the reliability of correspondences. By employing an alternating optimization strategy, the module progressively updates the rotation and translation parameters.} This design enables IGASA to adapt to diverse point cloud structures and complex transformations, significantly improving registration accuracy while maintaining computational efficiency.

Our method's efficacy is rigorously validated across three widely recognized benchmark datasets: 3DMatch~\cite{zeng20173dmatch},3DLoMatch~\cite{huang2021predator}, KITTI~\cite{geiger2013vision}, and nuScenes~\cite{caesar2020nuscenes}. Experimental results consistently demonstrate that our method substantially outperforms state-of-the-art methods, achieving superior registration accuracy and robustness even under challenging conditions. As illustrated in~\cref{figurelabel}, IGASA achieves the highest Inlier Ratio across various overlapping scenes, underscoring its robust performance.

Beyond accuracy, the computational efficiency of IGASA is a key aspect of its design. The framework is engineered to strike an optimal balance between complexity and performance, making it well-suited for real-time applications. IGASA is optimized for rapid convergence within a minimal number of iterations, ensuring overall efficiency without compromising its high accuracy.


Our main contributions are summarized as follows:
\begin{itemize}
% \item We introduce the HCLA module, a novel component engineered to leverage skip attention for precisely aligning multi-resolution features, ensuring both local and global geometric consistency across point cloud structures.
% \item A key advancement in our IGAR module. This iterative refinement strategy effectively utilizes potent \rev{spatial geometric consistency}, in conjunction with an alternating optimization strategy, to actively suppress outliers and substantially enhance the accuracy of pose estimation.
% \item We design an innovative HPA. This architecture seamlessly integrates highly efficient multi-scale feature extraction with robust and scalable registration capabilities, making it exceptionally well-suited for tackling complex real-world scenarios.

\item We introduce the HCLA module, a novel component engineered to leverage skip attention for precisely aligning multi resolution features, ensuring both local and global geometric consistency across point cloud structures.

\item \rev{We propose the IGAR module, an iterative refinement strategy that utilizes spatial geometric consistency. By employing an alternating optimization method, it actively suppresses outliers and significantly enhances the precision of the final pose estimation.}

\item \rev{We design an innovative HPA framework that seamlessly integrates efficient multi-scale feature extraction with robust registration capabilities, making the model exceptionally well suited for complex real world scenarios.}

\item \rev{We conduct extensive evaluations on widely recognized benchmarks, including 3D(Lo)Match, KITTI, and nuScenes. Experimental results demonstrate that our proposed IGASA significantly outperforms state of the art methods, achieving superior accuracy and robustness.}

\end{itemize}


==> sec/2_related.tex <==
\section{RELATED WORK}
\label{sec:formatting}



\subsection{Point Cloud Registration}

\rev{PCR is pivotal in 3D computer vision, underpinning applications such as autonomous driving and SLAM~\cite{bai2021pointdsc, jiang2024gtinet}. Traditionally, optimization based methods, exemplified by the ICP algorithm~\cite{sharp2002icp} and its variants~\cite{jost2002fast, yang2015go}, rely on nearest neighbor search to iteratively minimize alignment errors. However, the reliance on spatial proximity renders the optimization objective inherently non convex. Consequently, these methods are highly susceptible to converging to local minima when confronted with large initial misalignments or sparse data~\cite{vizzo2023kiss}, necessitating precise initialization to guarantee convergence.}

\rev{Recent advancements in deep learning have shifted focus toward end-to-end learning frameworks. While early methods utilized local descriptors~\cite{gojcic2019perfect,choy2019fully}, state-of-the-art methods increasingly leverage Transformer architectures to model long-range dependencies and global context~\cite{qin2022geometric,lu2019deepvcp,xie2024hecpg}. Despite their proficiency in handling low-overlap scenarios, these deep architectures often encounter a critical limitation known as the semantic gap. As network depth increases to capture high-level semantics, fine-grained geometric details are frequently diluted due to aggressive downsampling operations. This loss of high-frequency cues complicates precise local alignment, particularly in complex scenes with varying point densities.}

\rev{To address these challenges, we propose the IGASA framework. Distinct from prior arts, our method bridges the semantic gap via a HCLA module that explicitly preserves multi-scale features. Furthermore, we integrate an IGAR module to dynamically enforce geometric consistency, ensuring robust and high-precision registration.}

\begin{figure*}[t]
  \centering
  \includegraphics[width=1\linewidth]{fig2.pdf}
  % \caption{The workflow overview of IGASA. Our approach adopts a hierarchical modular framework consisting of three sequential modules: HPA module, HCLA-based feature extraction module, and IGAR module. The HPA module extracts point cloud features across three levels; The HCLA module utilizes a skip attention mechanism to accurately align and fuse features of varying resolutions; The IGAR module conducts iterative geometric optimization on initially matched corresponding points.}
  \caption{\rev{The overview of the proposed IGASA framework. The pipeline operates in three stages. \textbf{(a)}, the HPA module processes the source $P$ and target $Q$ inputs to construct a hierarchical feature pyramid ($F_{ordinary}, F_{minor}, F_{primary}$) with progressively expanding receptive fields. \textbf{(b)}, the HCLA module performs coarse matching by utilizing the SGIRA to fuse global semantics with local geometry, followed by the SAIGA for feature refinement. \textbf{(c)}, the IGAR module executes the fine registration phase, where an iterative optimization loop (repeated $N$ times) dynamically updates correspondence weights to suppress outliers and estimate the final transformation $\{R, t\}$.}}
  \label{figurelabe2}
  \vspace{-5mm}
\end{figure*}



\subsection{Transformer and Skip-Attention Mechanism}

\rev{Transformer-based architectures have significantly advanced point cloud registration by leveraging self-attention to capture long-range dependencies and global context~\cite{qin2022geometric, yew2022regtr, xu2024igreg}. These models demonstrate robustness in handling complex spatial variations and noise. However, standard self-attention mechanisms primarily focus on intra-layer interactions, often neglecting the effective integration of multi-resolution features required for fine-grained alignment.}

\rev{Although traditional skip connections~\cite{agarwal2023attention, wen2020point},~\cite{wang2024neighborhood, yuan2023egst} attempt to mitigate this by transferring high-resolution features from shallow layers, they typically rely on naive fusion strategies such as concatenation or summation~\cite{chen2019multi, horache20213d}. These methods suffer from a critical semantic gap, where the discrepancy between low-level geometric cues ($e.g.,$ edges, local density) and high-level semantic embeddings leads to suboptimal feature fusion. Consequently, critical geometric details are often diluted during the fusion process, limiting the model's precision~\cite{wang2022improving, yuan2023pointmbf}.}

\rev{To bridge this gap, we introduce a skip-attention mechanism inspired by multi-scale fusion strategies~\cite{lin2022ds, zhou2022sewer}. Unlike direct feature transfer, our method utilizes global semantic information derived from deep layers to dynamically modulate high-resolution features within a pyramid architecture. By computing cross-layer attention weights, the module selectively emphasizes geometrically relevant regions while suppressing noise and irrelevant background.}


% \subsection{\rev{Coarse-to-Fine Refinement}}

% Pyramid architectures facilitate robust multi-scale feature extraction~\cite{ghiasi2019fpn},~\cite{nie2022pyramid,yuan2024learning}, particularly for tasks requiring the integration of fine local details with global context. \rev{Recent multi-stage frameworks like PYRF-PCR~\cite{zhang2023pyrf} have further validated the efficacy of coarse-to-fine strategies in complex outdoor environments.} By employing multi-resolution strategies, these frameworks effectively model the spatial hierarchies and inherent variability of unstructured point clouds.

% Prior research, including Pyramid Point Networks~\cite{hui2021pyramid} and PF-Net~\cite{huang2020pf}, has demonstrated that multi-scale fusion significantly enhances structural understanding. Conventional methods~\cite{yu2021cofinet,xie2024hecpg},~\cite{thomas2019kpconv,huang2022imfnet} typically utilize pyramid structures to process data at varying resolutions, ensuring the capture of both local geometry and global context. Similarly, Transformer-based approaches such as GeoTransformer~\cite{qin2022geometric}, EGST~\cite{she2024pointdifformer}, and RegTR~\cite{yew2022regtr} leverage hierarchical designs to model long-range dependencies across scales. These architectures bolster registration accuracy by fusing semantic information with localized features.

% \rev{In this work, we propose an HPA tailored for point cloud registration. The HPA adopts a top-down structure that progressively refines feature representations from coarse to fine scales. At each level, the network extracts multi-granular features, integrating high-level semantic abstractions with low-level geometric details.}

\subsection{\rev{Coarse-to-Fine Refinement}}

\rev{Coarse-to-Fine strategies have become the paradigm for robust registration, leveraging pyramid architectures~\cite{ghiasi2019fpn},~\cite{nie2022pyramid,gong2025med} to resolve scale ambiguity. Particularly, recent frameworks like PYRF-PCR~\cite{zhang2023pyrf} have validated the efficacy of this strategy in complex outdoor environments by progressively refining poses from low to high resolution.}

\rev{Existing methods utilize these hierarchical designs to establish correspondences. For instance, methods like CoFiNet~\cite{yu2021cofinet} and KPConv-based architectures~\cite{thomas2019kpconv,huang2022imfnet} use multi-scale fusion to ensure the capture of both local geometry and global context. Similarly, Transformer-based methods such as GeoTransformer~\cite{qin2022geometric}, EGST~\cite{she2024pointdifformer}, and RegTR~\cite{yew2022regtr} leverage hierarchical dependencies to bolster coarse matching accuracy. However, the subsequent refinement stage in these methods often relies on RANSAC or hard-thresholding techniques to filter outliers. These explicit rejection strategies can be computationally expensive and sensitive to noise, often discarding valid correspondences in low-overlap regions.}

\rev{In contrast to these hard-decision methods, we propose the IGAR module. Instead of relying on noisy normal estimation or hard pruning, IGAR employs a dynamic geometric consistency weighting strategy. This acts as a soft suppression mechanism that iteratively down-weights inconsistent pairs, providing a more robust solution to outlier rejection in challenging, non-uniform environments.}

==> sec/3_method.tex <==
\section{METHODS}

\subsection{Overview}
\rev{In this section, we introduce the proposed IGASA framework. Our method are illustrated in the \cref{figurelabe2}, the proposed IGASA framework aligns the source point cloud $P$ and target $Q$ through a three-stage pipeline. Initially, the HPA module constructs a multi-scale representation by leveraging Kernel Point Convolution (KPConv) to extract features at $F_{primary}$, $F_{minor}$, and $F_{ordinary}$. Subsequently, the HCLA module integrates the extracted features using a cross-layer attention mechanism. This process utilizes global semantics from $F_{primary}$ to strategically guide the refinement of $F_{minor}$, outputting geometry optimized features $F_{minor}^{++}$ that are used to establish robust coarse correspondences. Finally, these preliminary matches are forwarded to the IGAR module, which performs fine-grained registration. This hierarchical design ensures a seamless data flow: HPA provides the multi-scale basis, HCLA aligns these features semantically, and IGAR refines the geometric alignment, forming a coarse-to-fine registration system.}



\subsection{Hierarchical Pyramid Architecture Module}
\rev{The proposed HPA is designed to efficiently extract multi-scale features from point cloud data, enhancing registration performance by integrating fine-grained local details. HPA constructs a multi-resolution representation through a progressive encoder framework, leveraging KPConv~\cite{thomas2019kpconv} in handling irregular point distributions.
The core mechanism of HPA adapts the formulation of KPConv which defines a set of $K$ learnable kernel points $\{\tilde{x}_k | k < K\}$ constrained within a sphere of radius $R_{in}$. For an arbitrary query point $p_i$ and its supporting neighborhood $N(p_i)$, the convolution weights are determined by the geometric correlation between the neighbors and the fixed kernel points. Formally, the feature aggregation $f(p_i)$ is computed as:
\begin{equation}
f(p_i) = \sum_{p_j \in N(p_i)} W(p_j - p_i) \cdot f(p_j),
\end{equation}
where $W(\cdot)$ denotes the kernel function defined by the linear correlation $max(0, 1 - \frac{\| (p_j - p_i) - \tilde{x}_k \|}{\sigma})$. The influence distance $\sigma$ and the kernel radius $R_{in}$ serve as the critical hyperparameters governing the receptive field, which we dynamically adjust to facilitate multi-scale feature extraction.}

\rev{To construct the feature pyramid, the HPA module employs a three-stage hierarchy comprising the ordinary, minor, and primary levels. We utilize a grid subsampling strategy where the voxel size, denoted as $dl$, is progressively increased to reduce point density while expanding the semantic scope. At the initial ordinary level, the input point cloud $P$ is processed with a base voxel size of $dl_0$. In this high-resolution layer, the KPConv influence radius is set to $R_{in} = 2.5 \cdot dl_0$, a configuration for capturing fine-grained local geometry and preserving detailed spatial relationships. Subsequently, the network transitions to the minor level, where grid subsampling is applied with a voxel size of $2 \cdot dl_0$, producing features that encapsulate semi-global structures while reducing computational redundancy.
Finally, at the primary level, the point cloud is downsampled to a coarse resolution of $4 \cdot dl_0$, with the convolution radius extended to $10.0 \cdot dl_0$. The resulting multi-scale feature set is expressed as:
\begin{equation}
    F_{\mathrm{multi}} = \left\{ F_{\mathrm{ordinary}}, F_{\mathrm{minor}}, F_{\mathrm{primary}} \right\}.
\end{equation}}

\rev{By systematically scaling the convolution radius commensurate with the sampling density, the HPA ensures that the network transition its receptive field from local geometric fidelity to global semantic coherence, yielding a hierarchical feature space suitable for the subsequent attention based alignment.}


% \subsection{Hierarchy Pyramid Architecture Module}

% The proposed Hierarchical Pyramid Architecture (HPA) is designed to efficiently extract multi-scale features from point cloud data, thereby enhancing registration performance by capturing both fine-grained local details and broader contextual information. HPA constructs a multi-resolution representation through progressive downsampling and convolution operations, which allows for handling point cloud data at different scales and levels of detail.

% The core mechanism of HPA leverages Kernel Point Convolution (KPConv) for feature extraction, combined with a hierarchical downsampling strategy. KPConv allows for adaptive convolution operations that capture local geometric features, while the hierarchical downsampling progressively reduces point cloud density to focus on broader semantic structures. For each point $p_k$, KPConv aggregates features from its neighborhood $N(p_k)$ using a weight function $W(p_i,p_k)$ that quantifies the geometric relationship between the center point $p_k$ and its neigobor $p_i$, alongside a geometric feature transformation $\psi(x(p_i),x(p_k))$. Formally, the output feature for $p_k$ can be expressed as:
% \begin{equation}
% f_{\mathrm{KPConv}}(p_k)
% = \sum_{p_i \in \mathcal{N}(p_k)}
% W\bigl(p_i,\,p_k\bigr)\,\psi\!\bigl(x(p_i),\,x(p_k)\bigr).
% \tag{1}
% \end{equation}

% HPA adopts a three-level pyramid: ordinary, minor, and primary to extract features across multiple scales. In each feature layer, KPConv is used to capture fine-grained local details. To the ordinary feature layer, the input point cloud $P$ is first processed at full resolution to capture fine-grained local geometry. KPConv produces high-resolution features $f_{ordinary}(p_i)$, preserving detailed spatial relationships between points:
% \begin{equation}
% \begin{split}
% f_{\mathrm{ordinary}}(p_i)    &= \sigma_{\mathrm{KPConv}}\left( x_{p_i}, W_{\mathrm{ordinary}} \right), \\
% \end{split}\tag{2}
% \end{equation}
% where $\sigma_{\mathrm{KPConv}}$ denotes the convolution and nonlinear activation, and $W_{\mathrm{ordinary}}$ represents the learnable parameters.

% To the minor feature layer, the point cloud is downsampled via voxel pooling or clustering to reduce density and computational load, producing a mid-level representation.  The further downsampling in the primary feature layer produces the lowest resolution point set, which enables the extraction of global features. KPConv at this level captures large-scale geometric patterns and long-range dependencies, which are essential for understanding the overall structure of the scene. 
% The calculation process are expressed as:
% \begin{equation}
% \begin{split}
% f_{\mathrm{minor}}(p_j)    &= \sigma_{\mathrm{KPConv}}\left( \varphi_{\mathrm{voxel}}(p_j), W_{\mathrm{minor}} \right), \\
% f_{\mathrm{primary}}(p_k)  &= \sigma_{\mathrm{KPConv}}\left( \varphi_{\mathrm{voxel}}(p_k), W_{\mathrm{primary}} \right),
% \end{split}\tag{3}
% \end{equation}
% where $\sigma_{\mathrm{KPConv}}$ denotes the convolution and nonlinear activation, $\varphi_{\mathrm{voxel}}$ is the downsampling function.
% This global perspective ensures that large-scale geometric patterns are adequately modeled. After these three stages, HPA produces a multi-scale feature set:
% \begin{equation}
%     F_{\mathrm{multi}} = \left\{ f_{\mathrm{ordinary}}, f_{\mathrm{minor}}, f_{\mathrm{primary}} \right\}, \tag{4}
% \end{equation}
% which encapsulates fine-grained local details, intermediate-scale contextual cues, and coarse global semantics. By systematically combining KPConv-based local feature extraction with hierarchical downsampling, HPA provides a detailed, well-rounded representation of point clouds, enabling more precise and efficient registration. 

\subsection{Hierarchical Cross-Layer Attention Module}

\rev{The HCLA module is designed as the core integration engine to bridge the semantic gap between multi-resolution features. While standard concatenation fuses features mechanically, it often fails to address the misalignment between global context and local geometry. To address this, HCLA introduces a structured mechanism composed of two specialized components: Skip-Guided Inter-Resolution Attention (SGIRA) and Skip-Augmented Intrinsic Geometric Attention (SAIGA).}

\rev{SGIRA acts as a semantic filter. It leverages the deep, globally-aware features from the primary layer as a guide to weigh the high-resolution features in the minor layer. This process ensures that the model focuses only on semantically relevant local details while suppressing ambiguous background noise caused by resolution differences. Following this cross-layer filtering, SAIGA functions as a geometric sharpener. It performs self-attention on the filtered features to reinforce their intrinsic spatial distinctiveness, ensuring that the final descriptors are robust to viewpoint changes.}

\rev{After alignment, HCLA applies a geometric consistency evaluation to filter coarse matches. The initial point pairs generated from low-resolution features are refined through hypothesized rigid transformations. Subsequently, a compatibility graph is constructed to assess geometric consistency by quantifying the error between pairs, and a $top$-$k$ selection strategy is employed to retain the most reliable point pairs, ensuring accurate correspondences for subsequent fine registration.}

% The HCLA mechanism enhances feature alignment by integrating global semantic information and optimizing geometric consistency. It consists of two key components: Skip-Guided Inter-Resolution Attention (SGIRA) and Skip-Augmented Intrinsic Geometric Attention (SAIGA).

% SGIRA facilitates the alignment of semantics and geometry between low- and high-resolution features, which uses a cross-layer attention mechanism. Low-resolution features $F_{primary}$ provide global semantic guidance, while high-resolution features $F_{minor}$ capture detailed local geometry. Both feature sets are mapped to a shared embedding space, and dynamic attention weights are computed based on semantic similarity (dot product), geometric consistency (Euclidean distance), and skip feature guidance.

% SAIGA focuses on optimizing geometric consistency within high-resolution features by modeling local point interactions. It uses self-attention, where semantic similarity is captured via dot product, and Euclidean distances compensate for the sparsity and irregularity of point clouds. This module employs a dynamic skip feedback mechanism that integrates cross-layer information, further refining attention weights based on intrinsic geometric properties.

% After alignment, HCLA applies a geometric consistency evaluation to filter coarse matches. The initial point pairs generated from low-resolution features are refined through hypothesized rigid transformations, and a compatibility graph is constructed to quantify the error between pairs. A compatibility graph is constructed to assess geometric consistency, with a $top$-$k$ selection strategy retaining the most reliable point pairs, ensuring accurate correspondences for subsequent fine registration.

\subsubsection{Skip-Guided Inter-Resolution Attention}

The SGIRA module is designed to facilitate the alignment of semantics and geometry between low and high resolution features using a cross-layer attention mechanism. The feature $F_{primary}$, representing global semantics, guides the fusion of high-resolution features $F_{minor}$, which capture detailed local geometry. 

\rev{To enhance this fusion, skip features from intermediate layers are incorporated to refine the distribution. While \cref{figurelabe2} (b) illustrates the logical flow of this feature integration, the specific mathematical implementation is detailed in \cref{figurelabe3}. We employ a Gated Fusion Mechanism at this interaction point, which utilizes parallel convolutional branches to dynamically weigh and combine features from different resolutions, ensuring that complementary information is effectively integrated.}
This mechanism first normalizes the input features to standardize their scale and distribution, improving the stability of subsequent operations. It then uses two convolutional branches to transform and gate the features. These branches are subsequently merged via a gating operation that computes adaptive weights, ensuring that the features from both resolutions are balanced appropriately. A residual adjustment step further enhances the features by correcting and refining them. Finally, a weighted fusion process combines these refined features, giving the final output a balanced and enriched representation.

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{fig3.pdf}
  \caption{Details of Gated Fusion Mechanism. $F_p^n$ and $F_q^n$ are preprocessed, passed through parallel convolutional layers, combined to form $F_t$, and then refined by a residual adjustment to produce $G_{\text{fusion}}$ for weighted fusion.}
  \label{figurelabe3}
  \vspace{-5mm}
\end{figure}
The core of SGIRA is its attention mechanism, which not only measures semantic similarity between low and high resolution features but also incorporates geometric consistency and skip-feature guidance. The calculation process is as follows: 
\begin{equation}
    S_{ij} = \frac{Q_i K_j^T}{\sqrt{d_a}},
\end{equation}
where $S_{ij}$ reflects how closely point $i$ aligns semantically with point $j$ and $\sqrt{d_a}$ is the scaling factor. To account for geometric alignment, we define a compensation term $R_{ij}$ to reflect spatial alignment. The equation is formulated:
$R_{ij} = -\frac{\| P_i - M_j \|^2}{\sigma^2}$,
where $P_i,M_j$ represent the coordinates of the two points in the three-dimensional space. 
In addition to this, a crucial step is the weighting of the distances through the skip mechanism. Following this, we can calculate the residual error through the use of the $A_{ij}$ coefficient and the Softmax function, which normalizes the computation by applying a weight to the spatial differences.
%, leading to the final approximation of the spatial assignment:
%$A_{ij} = \text{Softmax}\left(S_{ij} + R_{ij} + \beta \cdot A_{\text{skip}} + b_{ij}\right)$.
Subsequently, we define the total residual function for optimization as:
$F_{\text{minor}}^{+} = \sum_{i=1}^{N_p} A_{ij} \cdot V_i$,
where $F_{\text{minor}}^{+}$ represents the low-frequency residual values influenced by the spatial distribution model. The residual function is given by:
\begin{equation}
F^{++}_{\text{minor}} 
= F^{+}_{\text{minor}}
+ \gamma \cdot \mathrm{SkipResidual}\!\Bigl(F^{+}_{\text{minor}},\,F_{\text{skip}}\Bigr),
\end{equation}
the term $\gamma$ scales the contribution of the skip residual component and $F_{\text{skip}}$ obtained directly from the HPA module through several skip connections.

Overall, the SGIRA module efficiently combines semantic, geometric, and skip-feature information, ensuring effective multi-scale feature fusion while maintaining computational efficiency and spatial consistency.

\subsubsection{Skip-Augmented Intrinsic Geometric Attention}

This module aims to optimize the geometric alignment within high-resolution point cloud features. SAIGA centers on refining local geometric structures. 
Starting with the feature $F^{+}_{\text{minor}}$, SAIGA performs feature projection, neighborhood alignment weight computation, and feature updates to iteratively improve feature alignment. After completing the feature projection step, the SAIGA module employs a self-attention mechanism that dynamically calculates pairwise weight distributions. The calculation of attention weights involves two key components: semantic similarity measurement and geometric distance compensation. Semantic similarity focuses on the interaction between the query vector $Q_{geo}$ and the key vector $K_{geo}$. By performing a scaled dot-product calculation, the module quantifies the correlation between each high-resolution point and its neighborhood points, as expressed by the formula:
\begin{equation}
S_{\text{geo}, ij} = \frac{Q_{\text{geo}, i} K_{\text{geo}, j}^T}{\sqrt{d_a}},
\end{equation}
where $\sqrt{d_a}$ represents the dimensionality of the query and key vectors, ensuring numerical stability during the computation. And the geometric distance weight models the contribution of the Euclidean distance between points $i$ and $j$ in the similarity computation, formulated as:
$R_{\text{geo}, ij} = -\alpha \| M_i - M_j \|^2$,
where $M_i,M_j$ denote the 3D coordinates of points $i$ and $j$, and $\alpha$ is a learnable hyperparameter that controls the influence of geometric distance.

By integrating the semantic similarity $S_{\text{geo}, ij}$ with the geometric distance compensation $R_{geo,ij}$, the SAIGA module calculates a comprehensive attention weight. Additionally, the combined attention weight is then normalized using the Softmax function, as described by:
$A_{\text{geo}, ij} = \text{Softmax}\left(S_{\text{geo}, ij} + R_{\text{geo}, ij} + \theta \cdot A_{\text{skip}}\right)$. 

Once the attention weights are computed, SAIGA performs a weighted feature aggregation over the value matrix $V_{geo}$ to update the high-resolution features. The final geometry-optimized feature representation is expressed as:
\begin{equation}
F^{++}_{\text{minor},i} 
= F^{+}_{\text{minor},i}
+ \sum_{j=1}^{N_m} A_{\text{geo}, ij} \cdot V_{\text{geo}, j},
\end{equation}
where $F^{++}_{\text{minor},i}$ represents the geometry-optimized feature of the $i-th$ high-resolution point. $F^{++}_{\text{minor},i}$ composed of the updated features for all points, serves as the final output of this step. The use of skip-augmented attention allows the model to preserve long-range dependencies while reinforcing local feature consistency.

Finally, by leveraging this attention-based feature refinement, the SAIGA module effectively yields high-resolution point representations.

\subsubsection{Superpoint matching module}

In the establishment of coarse matching relationships, we leverage the low-resolution features output to construct preliminary correspondences across the global scope. The feature representations of the source and target point clouds are denoted as $F_{\text{src}}^{(1)} = \bigl\{\, f_{\text{src},j}^{(1)} \in \mathbb{R}^d\bigr\}$ and $F_{\text{tar}}^{(1)} = \bigl\{\, f_{\text{tar},j}^{(1)} \in \mathbb{R}^d\bigr\}$, respectively. To establish these initial correspondences, for any given source point $p^{(1)}_{src,j}$, we employ a nearest neighbor search to identify the target point $p^{(1)}_{tar,k}$. \rev{The similarity between the features of the two points is defined by the Euclidean distance:
$\text{Sim}(f_{\text{src}, j}^{(1)}, f_{\text{tar}, k}^{(1)}) = \| f_{\text{src}, j}^{(1)} - f_{\text{tar}, k}^{(1)} \|_2$.
Consequently, the target point with the minimum distance is selected as the match, formalized as $p_{\text{src}, j}^{(1)} \leftrightarrow p_{\text{tar}, k}^{(1)}$,where $k = \arg\min_{k} \bigl\| f_{\text{src}, j}^{(1)} - f_{\text{tar}, k}^{(1)} \bigr\|_2$.}

% Here, the target point with the minimal distance is selected as the matching counterpart to the source point. The target point exhibiting the smallest distance is selected as the corresponding match, formalized mathematically as:
% \begin{equation}

% \quad,\text{where}\quad
% .
% \end{equation}

Through this process, a set of preliminary matching point pairs is generated, expressed as:
$C^{(1)} = \left\{ p_{\text{src}, j}^{(1)}, p_{\text{tar}, k}^{(1)} \right\} \quad j = 1, 2, 3, \dots, N_{\text{src}}$, 
where $N_{\text{src}}$ denotes the total number of points in the source point cloud. We use a $top$-$k$ selection strategy based on a geometric consistency score to filter out erroneous matches from the coarse matching set $C^{(1)}$. The geometric consistency score is defined by an initial transformation matrix $T_{init}=(R_{init},t_{init})$. For any given point pair $p_{\text{src},j}^{(1)}$ and $p_{\text{tar}, k}^{(1)}$, the consistency score is calculated as:
\begin{equation}
    S_{\text{geo}}^{(1)} \left( p_{\text{src}, j}^{(1)}, p_{\text{tar}, j}^{(1)} \right) 
    = \exp \Bigl( - \frac{\left\| R_{\text{init}} p_{\text{src}, j}^{(1)} + t_{\text{init}} - p_{\text{tar}, j}^{(1)} \right\|_2^2}{\sigma^2} \Bigr),
\end{equation}
where $\sigma$ is a scale parameter that modulates the sensitivity of the score. The use of the exponential function ensures that small misalignments are tolerated while large discrepancies lead to a rapid decline in the consistency score. 

Upon computing the geometric consistency scores for all point pairs $\bigl(p_{\text{src}, j}^{(1)}, p_{\text{tar}, j}^{(1)}\bigr) \in C^{(1)}$, the pairs are sorted in descending order based on their scores. Then retains the $k$ highest-scoring pairs, formalized as:
$\widetilde{C}^{(1)} = top$-$k\:\!\bigl(C^{(1)}, S_{\text{geo}}^{(1)}\bigr)$,
which refined subset $\widetilde{C}^{(1)}$ ensures that only the most geometrically consistent matches are preserved. This refined matching set serves as a robust foundation for subsequent fine registration processes by effectively filtering out outliers and erroneous matches. 

\subsection{Iterative Geometry-Aware Refinement Module}

The IGAR module functions within the fine matching phase, facilitating high-precision pose estimation through the integration of spatial geometric cues and an alternating optimization framework. \rev{Specifically, the module incorporates a Dynamic Geometric Consistency mechanism. This strategy prioritizes geometrically consistent pairs by adaptively weighting correspondences based on their spatial fidelity, thereby mitigating the influence of outliers. To quantify geometric reliability, let the source and target point clouds be denoted by the sets $P_{\mathrm{src}} = \{p_{\mathrm{src}, j}^{(1)}\}$ and $P_{\mathrm{tar}} = \{p_{\mathrm{tar}, j}^{(1)}\}$, initialized with a transformation $T_{\mathrm{init}}=(R_{\mathrm{init}},t_{\mathrm{init}})$.} We assign a consistency weight $w_{ij}$ to each correspondence pair, initially derived from the Euclidean spatial discrepancy:
\begin{equation}
w_{ij}^{(1)} = \exp \Bigl( - \frac{\| p_{\mathrm{src}, j}^{(1)} - p_{\mathrm{tar}, j}^{(1)} \|^2}{\sigma^2} \Bigr),
\end{equation}
where $\sigma^2$ denotes the scale parameter regulating sensitivity to spatial deviations. Through iterative refinement, both the weights and the transformation parameters are dynamically updated. \rev{At the $k$-th iteration, the weight is re-evaluated to reflect the instantaneous alignment error:
\begin{equation}
\begin{split}
w_{ij}^{(k)} ={} & \exp\Bigl(-\frac{\bigl\lVert p_{\mathrm{tar},j}^{(1)} - \bigl(R^{(k)} p_{\mathrm{src},j}^{(1)} + t^{(k)}\bigr)\bigr\rVert^2}{\sigma^2}\Bigr) \\
& \times \mathbb{I}\bigl[\bigl\lVert p_{\mathrm{tar},j}^{(1)} - \bigl(R^{(k)} p_{\mathrm{src},j}^{(1)} + t^{(k)}\bigr)\bigr\rVert < \tau \bigr],
\end{split}
\end{equation}
where $R^{(k)}$ and $t^{(k)}$ represent the optimized rotation and translation at iteration $k$, and $\mathbb{I}_{[\cdot]}$ serves as an indicator function that thresholds large deviations to exclude gross outliers. This formulation effectively embeds spatial distribution constraints into the optimization objective:
\begin{equation}
E(R, t) = \sum_{(i,j)\in \mathcal{C}} w_{ij}^{(k)} \| R p_{\mathrm{src},j}^{(1)} + t - p_{\mathrm{tar},j}^{(1)} \|_2^2.
\end{equation}}

To resolve this objective, we employ a weighted pseudo-center optimization strategy. The process commences by computing the weighted centroids of the source and target point sets, $\bar{p}_{\mathrm{src}}$ and $\bar{p}_{\mathrm{tar}}$, defined as:
\rev{\begin{equation}
\bar{p}_{\mathrm{src}}
= \frac{\displaystyle \sum_{(i,j)\in \mathcal{C}} w_{ij}^{(k)}\,p_{\mathrm{src},j}^{(1)}}
        {\displaystyle \sum_{(i,j)\in \mathcal{C}} w_{ij}^{(k)}}
\enspace,\enspace
\bar{p}_{\mathrm{tar}}
= \frac{\displaystyle \sum_{(i,j)\in \mathcal{C}} w_{ij}^{(k)}\,p_{\mathrm{tar},j}^{(1)}}
        {\displaystyle \sum_{(i,j)\in \mathcal{C}} w_{ij}^{(k)}}.
\end{equation}}

\rev{Subsequently, a weighted cross-covariance matrix $C \in \mathbb{R}^{3 \times 3}$ is constructed to encapsulate the structural correlation between the point sets, focusing the alignment on regions with high geometric consistency:
\begin{equation}
C
= \sum_{(i,j)\in \mathcal{C}} w_{ij}^{(k)}\,\bigl(p_{\mathrm{src},j}^{(1)} - \bar{p}_{\mathrm{src}}\bigr)\,\bigl(p_{\mathrm{tar},j}^{(1)} - \bar{p}_{\mathrm{tar}}\bigr)^{T}.
\end{equation}}

\rev{By performing SVD on the covariance matrix $C = U \Sigma V^T$, the optimal rotation matrix $R^*$ and translation vector $t^*$ are derived as:
\begin{equation}
R^* = VU^T, \quad t^* = \bar{p}_{\mathrm{tar}} - R^* \bar{p}_{\mathrm{src}}.
\end{equation}}

Ultimately, the IGAR module outputs a high-precision pose transformation matrix $T^*=[R^*, t^*]$. This transformation enables precise alignment of $P_{\mathrm{src}}$ with $P_{\mathrm{tar}}$, achieving robust and accurate registration.

\subsection{Loss function}
%is designed to supervise key modules of point cloud registration: coarse(fine) matching, keypoint matching, and dense registration.
Our loss function $\mathcal{L}_{\text{total}}$ is composed of a matching loss function $\mathcal{L}_{\text{mat}}$, a keypoint loss function $\mathcal{L}_{\text{key}}$ and a dense loss function $\mathcal{L}_{\text{den}}$.

\textbf{Matching Loss.} Given a set $C$ of coarse correspondences, where each pair $(i,j)\in C$ is assigned an overlap weight $w_{ij}$, let $P^{(l)}_{ij}$ denote the matching probability. The hierarchical loss is formulated as:
\begin{equation}
\mathcal{L}_p = -\frac{1}{L} \sum_{l=1}^{L} \sum_{(i,j)\in C} w_{ij} \log \bigl(P_{ij}^{(l)}\bigr),
\end{equation}
which ensures that the predicted matching probabilities at multiple layers are consistent with the given overlap weights $w_{ij}$. This structure allows the network to learn representations at different scales and provides a gradual refinement of matches.
For the final matching probabilities $P_{ij}$, we enforce supervision using a weighted cross-entropy loss $\mathcal{L}_c$:

\begin{multline}
\mathcal{L}_{c} = - \frac{1}{\sum_{(i,j)\in C} \omega_{ij}} \sum_{(i,j)\in C} \omega_{ij} \log P_{ij} \\
\shoveleft{- \frac{1}{|N_X|} \sum_{k\in N_X} \log\Bigl(1 - \hat{\omega}^X_k\Bigr) + \frac{1}{|N_Y|} \sum_{k\in N_Y} \log\Bigl(1 - \hat{\omega}^Y_k\Bigr),}
\end{multline}
where $N_x$ and $N_y$ denote the sets of semi-dense nodes in the source and target clouds that are not involved in any correspondence, with $\hat{w}^X_k$ and $\hat{w}^Y_k$ representing their estimated overlap probabilities. The overlap weight $\omega_{ij}$ is computed based on a spherical neighborhood of radius $r$. The matching loss $\mathcal{L}_{\text{mat}}=\lambda_p \mathcal{L}_p + \lambda_c \mathcal{L}_c$, where $\lambda_p,\lambda_c$ are used to balance the terms. This dual aspect ensures that the network distinguishes between true matches and outliers, effectively reducing false correspondences.

\textbf{Keypoint Matching Loss.} For each valid keypoint correspondence $(x,x^+)$ with descriptors $d_x$ and $d_{x^+}$, we use a learnable weight matrix $W$ to compute similarity. An InfoNCE-style loss maximizes the similarity for true pairs while suppressing the negatives (denoted by the set $N_x$):

\begin{equation}
\begin{split}
\mathcal{L}_f &= -\mathbb{E}_{(x, x^+, N_x)}  \\
  &\Bigl[\log \frac{
  \exp\bigl(\langle d_x, W d_{x^+} \rangle\bigr)
  }{
  \exp\bigl(\langle d_x, W d_{x^+} \rangle\bigr)
  + \sum_{n \in N_x} \exp\bigl(\langle d_x, W d_n \rangle\bigr)
  } 
  \Bigr].
\end{split}
\end{equation}


For each keypoint $x$ with its predicted correspondence $\hat{y}$(extracted from its local patch $C_x$), 
we use an $\mathcal{L}_k$ loss to penalize positional errors:
\begin{equation}
\mathcal{L}_k = \mathbb{E}_{(x, \hat{y})}\bigl\|R\,x + t - \hat{y}\bigr\|^2.
\end{equation}

Each predicted correspondence is also assigned a confidence score $s$. We supervise these scores using a binary cross-entropy loss, where the ground truth label is 1 if $\| R x + t - \hat{y}\|\le\tau$. (with $\tau$ as a predefined threshold):
\begin{equation}
\mathcal{L}_i = -\mathbb{E}_{(x, \hat{y})} \left[ y \log s + (1 - y) \log (1 - s) \right].
\end{equation}

The keypoint matching loss function $\mathcal{L}_{\text{key}}= \lambda_f \mathcal{L}_f + \lambda_k \mathcal{L}_k + \lambda_i \mathcal{L}_i$.
The combination of these losses, each balanced by weights $\lambda_f,\lambda_k,\lambda_i$, ensures that both descriptor similarity and geometric accuracy are maintained.

\textbf{Dense Registration Loss.} To ensure the overall transformation is accurate, we supervise the dense registration phase by constraining the translation and rotation parameters:
$\mathcal{L}_t = \|\hat{t} - t\|^2,
\mathcal{L}_r = \|\hat{R}^T R - I\|_F^2,$
where $I$ is the $3*3$ identity matrix and the $F$ norm enforces closeness of the estimated rotation to the ground truth. The dense registration loss function $\mathcal{L}_{\text{den}}= \lambda_t \mathcal{L}_t + \lambda_r \mathcal{L}_r$, where $\lambda_t,\lambda_r$ are the weight of loss, guarantees that the final registration is not only locally accurate but also globally consistent.

The overall loss is a weighted combination of all the components: 
\begin{equation}
\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{mat}}+\mathcal{L}_{\text{key}}+\mathcal{L}_{\text{den}}.
\end{equation}

This comprehensive loss formulation ensures robust training by addressing errors at various levels, including coarse matching, fine keypoint alignment, and dense global registration. By penalizing deviations at each stage, the proposed loss significantly enhances the accuracy and stability of the overall registration framework.

\begin{figure*}[t]
  \centering
  \includegraphics[width=1\linewidth]{fig4.pdf}
  \caption{The result of IGASA on 3D(Lo)Match. We visualized some of the scenes in the dataset. The first row shows the initial arrangement of the two point clouds in their raw, unaligned positions.The second row displays the registration result predicted by our model.}
  \label{figurelabe4}
  \vspace{-5mm}
\end{figure*}

==> sec/4_experiment.tex <==
\section{EXPERIMENT}
\subsection{Experiment details}

\rev{The proposed IGASA framework is implemented in PyTorch. For the HPA module, the feature dimensions for the three pyramid levels ($F_{ordinary}, F_{minor}, F_{primary}$) are set to 64, 128, and 256, respectively. This progressive increase in channel depth ensures the capture of rich semantic abstractions. The kernel influence radius $R_{in}$ for KPConv is dynamically scaled as $2.5 \times dl$, where $dl$ is the voxel size at each level.
In the HCLA module, we employ a multi-head attention mechanism with 4 heads, where each head has a dimension of 64. The SGIRA and SAIGA units are stacked 1 time to balance computational efficiency with feature alignment performance.
For the IGAR module, we empirically set the number of iterations to $N=5$, which provides sufficient stability for the dynamic weight update mechanism without incurring excessive computational overhead.}

\rev{We evaluate our method on both indoor and outdoor benchmarks. For the 3DMatch and 3DLoMatch indoor datasets, raw point clouds are downsampled using a voxel size of 0.025m. To prevent overfitting, we apply data augmentation during training, including random rotations around arbitrary axes and random scaling. For the KITTI and nuScenes outdoor benchmarks, considering the sparsity of LiDAR data, we use a larger voxel size of 0.3m.}

\rev{The model is trained on a single NVIDIA RTX 3090 GPU using the AdamW optimizer with an initial learning rate of $10^{-4}$ and weight decay of $10^{-4}$. The learning rate is decayed by a factor of 0.95 every epoch. We train the model for 15 epochs on 3DMatch, 30 epochs on KITTI, and 10 epochs on nuScenes. The batch size is set to 1. For detailed loss weight configurations and specific augmentation parameters, please refer to the Supplementary Material}.

% We evaluate IGASA on indoor 3D(Lo)Match benchmarks and outdoor KITTI, nuScenes benchmark. The implementation details are based on PyTorch and trained on an NVIDIA RTX 3090 GPU. Our Network is trained using an AdamW optimizer with a batch size of 1 and the weight decay rate is set to $10^{-6}$. The model is trained for 15 epochs on 3DMatch, 30 epochs on KITTI and 10 epochs on nuScenes. The learning rate starts from $10^{-4}$ and decreases the learning rate to 90\% every five steps, with gradients clipped at a norm of 0.5 during back propagation. We set $\lambda_p=\lambda_f=\lambda_i=1,\lambda_t=5,\lambda_r=20,$  $\lambda_c=1,\lambda_k=10$ for 3DMatch and $\lambda_c=0.2,\lambda_k=1$ for KITTI and nuScenes.

\begin{table*}[t]
\centering
%\scriptsize % This reduces the font size for the table
\caption{Evaluation results of our method on 3DMatch and 3DLoMatch datasets. Optimal results are highlighted in bold, with runner-up results indicated by an underline.}
\label{table1}
\renewcommand{\arraystretch}{0.88}
\resizebox{0.8\textwidth}{!}{ % Resizing the table to fit the single column width
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
\toprule % 最上方的加粗线
\ &\multicolumn{5}{c|}{3DMatch} & \multicolumn{5}{c}{3DLoMatch} \\
\# Samples & \multicolumn{1}{c}{5000} & \multicolumn{1}{c}{2500} & \multicolumn{1}{c}{1000} & \multicolumn{1}{c}{500} & \multicolumn{1}{c|}{250} & \multicolumn{1}{c}{5000} & \multicolumn{1}{c}{2500} & \multicolumn{1}{c}{1000} & \multicolumn{1}{c}{500} & 250 \\
\midrule
\multicolumn{11}{c}{\textit{Feature Matching Recall (\%) }$\uparrow$} \\
\midrule
% PerfectMatch~\cite{gojcic2019perfect} & 95.0 & 94.3 & 92.9 & 90.1 & 82.9 & 63.6 & 61.7 & 53.6 & 45.2 & 34.2 \\
FCGF~\cite{choy2019fully} & 97.4 & 97.3 & 97.0 & 96.7 & 96.6 & 76.6 & 75.4 & 74.2 & 71.7 & 67.3 \\
% D3Feat~\cite{bai2020d3feat} & 95.6 & 94.3 & 95.6 & 94.3 & 91.0 & 66.7 & 64.7 & 61.6 & 60.0 & 56.6 \\
% SpinNet~\cite{ao2021spinnet} & 97.6 & 97.2 & 96.8 & 95.5 & 96.5 & 75.3 & 74.9 & 72.5 & 70.0 & 63.6 \\
Predator~\cite{huang2021predator} & 96.6 & 96.6 & 96.5 & 96.3 & 95.3 & 78.6 & 76.7 & 75.7 & 75.7 & 72.9 \\
YOHO~\cite{wang2022you} & \textbf{98.2} & 97.6 & 97.5 & 97.7 & 96.0 & 79.4 & 78.1 & 76.3 & 73.8 & 69.1 \\
CoFiNet~\cite{yu2021cofinet} & \underline{98.1} & \underline{98.3} & \underline{98.1} & 98.2 & 98.3 & 83.1 & 83.5 & 83.3 & 83.1 & 82.6 \\
GeoTransformer~\cite{qin2022geometric} & 97.9 & 97.9 & 97.9 & 97.9 & 97.6 & 88.3 & 88.6 & 88.8 & \underline{88.6} & \underline{88.3} \\
PCR-CG~\cite{zhang2022pcr} & 97.4 & 97.5 & 97.7 & 97.3 & 97.6 & 80.4 & 82.2 & 82.6 & 83.2 & 82.8 \\
OIF-Net~\cite{yang2022one} & \underline{98.1} & 98.1 & 97.9 & \underline{98.4} & \underline{98.4} & 84.6 & 85.2 & 85.5 & \underline{88.6} & 87.0 \\
RoITr~\cite{yu2023rotation} & 98.0 & 98.0 & 97.9 & 98.0 & 97.9 & \textbf{89.6} & \textbf{89.6} & \textbf{89.5} & \textbf{89.4} & \textbf{89.3} \\
SIRA-PCR~\cite{chen2023sira} & \textbf{98.2} & \textbf{98.4} & \textbf{98.4} & \textbf{98.5} & \textbf{98.5} & \underline{88.8} & \underline{89.0} & \underline{88.9} & \underline{88.6} & 87.7 \\
IGASA (\textit{ours}) & \textbf{98.2} & 97.8 & 97.8 & 97.9 & 97.8 & 82.1 & 80.5 & 80.5 & 80.5 & 80.4 \\
\midrule
\multicolumn{11}{c}{\textit{Registration Recall (\%)} $\uparrow$} \\
\midrule
% PerfectMatch~\cite{gojcic2019perfect} & 78.4 & 76.2 & 71.4 & 67.6 & 50.8 & 33.0 & 29.0 & 23.7 & 11.0 & 15.9 \\
FCGF~\cite{choy2019fully} & 85.1 & 83.4 & 82.7 & 81.6 & 76.6 & 74.4 & 70.4 & 67.2 & 63.4 & 61.4 \\
% D3Feat~\cite{bai2020d3feat} & 81.6 & 84.5 & 83.4 & 82.7 & 77.9 & 69.4 & 60.2 & 58.5 & 51.6 & 42.6 \\
% SpinNet~\cite{ao2021spinnet} & 86.6 & 85.8 & 85.5 & 83.5 & 79.7 & 68.9 & 59.6 & 56.8 & 50.0 & 49.1 \\
Predator~\cite{huang2021predator} & 89.0 & 89.9 & 90.6 & 88.5 & 86.6 & 61.2 & 61.2 & 62.4 & 60.8 & 58.1 \\
YOHO~\cite{wang2022you} & 90.8 & 90.3 & 89.1 & 88.6 & 84.5 & 67.5 & 68.0 & 62.2 & 63.4 & 61.9 \\
CoFiNet~\cite{yu2021cofinet} & 92.0 & 91.8 & 91.8 & 91.4 & 91.2 & 75.0 & \underline{74.8} & 74.2 & 74.1 & 73.5 \\
GeoTransformer~\cite{qin2022geometric} & 92.0 & 91.8 & 91.1 & 91.4 & 92.0 & \underline{75.5} & \underline{74.8} & 74.6 & \underline{74.6} & \underline{75.3} \\
PCR-CG~\cite{zhang2022pcr} & 89.4 & 90.7 & 90.0 & 88.7 & 86.8 & 66.3 & 67.2 & 69.0 & 68.5 & 65.0 \\
OIF-Net~\cite{yang2022one} & 92.4 & 91.9 & 91.8 & 91.4 & 91.0 & 74.7 & \underline{74.8} & \underline{74.8} & 74.2 & 73.6 \\
RoITr~\cite{yu2023rotation} & 91.9 & 91.7 & 91.8 & 91.4 & 91.0 & 74.7 & \underline{74.8} & \underline{74.8} & 74.2 & 73.6 \\
\rev{FeatSync~\cite{hu2024featsync}} & 90.2 & 90.3 & 90.6 & 91.2 & 91.1 & - & - & - & - & - \\
SIRA-PCR~\cite{chen2023sira} & \underline{93.6} & \underline{93.9} & \underline{93.9} & \underline{92.7} & \underline{92.4} & 73.5 & 73.9 & 73.0 & 73.4 & 71.1 \\
IGASA (\textit{ours}) & \textbf{94.6} & \textbf{94.5} & \textbf{94.5} & \textbf{94.4} & \textbf{94.3} & \textbf{76.5} & \textbf{76.5} & \textbf{76.3} & \textbf{76.4} & 
\textbf{76.4} \\
\midrule
\multicolumn{11}{c}{\textit{Inlier Ratio (\%) }$\uparrow$} \\
\midrule
% PerfectMatch~\cite{gojcic2019perfect} & 36.0 & 32.5 & 26.4 & 21.5 & 16.4 & 11.4 & 10.1 & 8.0 & 6.4 & 4.8 \\
FCGF~\cite{choy2019fully} & 56.8 & 54.1 & 48.7 & 42.5 & 34.1 & 21.4 & 20.0 & 17.2 & 14.8 & 11.6 \\
% D3Feat~\cite{bai2020d3feat} & 39.0 & 38.8 & 40.4 & 41.5 & 41.8 & 13.2 & 13.1 & 14.0 & 14.6 & 15.0 \\
% SpinNet~\cite{ao2021spinnet} & 47.5 & 44.7 & 39.4 & 33.9 & 27.6 & 20.5 & 19.0 & 16.3 & 13.8 & 11.1 \\
Predator~\cite{huang2021predator} & 58.0 & 58.4 & 57.1 & 54.1 & 49.3 & 26.7 & 28.1 & 28.3 & 27.5 & 25.8 \\
YOHO~\cite{wang2022you} & 64.4 & 60.7 & 55.7 & 46.4 & 41.2 & 25.9 & 23.3 & 22.6 & 18.2 & 15.0 \\
CoFiNet~\cite{yu2021cofinet} & 49.8 & 51.2 & 51.9 & 52.2 & 52.2 & 24.4 & 25.9 & 26.7 & 26.8 & 26.9 \\
GeoTransformer~\cite{qin2022geometric} & 71.9 & 75.2 & 76.0 & 82.2 & 85.1 & 43.5 & 45.3 & 46.2 & 52.9 & 57.7 \\
OIF-Net~\cite{yang2022one} & 62.3 & 65.2 & 66.8 & 67.1 & 67.5 & 27.5 & 30.0 & 31.2 & 32.6 & 33.1 \\
RoITr~\cite{yu2023rotation} & \underline{82.6} & \underline{82.8} & 83.0 & 83.0 & 83.0 & \underline{54.3} & \underline{54.6} & 55.1 & 55.2 & 55.3 \\
\rev{OT-CA~\cite{guo2024learning}} & 59.5 & 61.5 & 60.9 & 61.7 & 61.7 & 30.5 & 30.6 & 30.5 & 34.9 & 30.2 \\
SIRA-PCR~\cite{chen2023sira} & 70.8 & 78.3 & \underline{83.7} & \underline{85.9} & \underline{87.4} & 43.3 & 49.0 & \underline{55.9} & \underline{58.8} & \underline{60.7} \\
IGASA (\textit{ours}) & \textbf{87.9} & \textbf{87.8} & \textbf{87.9} & \textbf{87.9} & \textbf{87.9} & \textbf{61.6} & \textbf{61.5} & \textbf{61.5} & \textbf{61.6} & \textbf{61.4} \\
\bottomrule % 底部加粗框线
\end{tabular}
}
\vspace{-5mm}
\end{table*}

\subsection{Indoor Benchmarks: 3DMatch \& 3DLoMatch}

% \begin{table}[t]
% \centering
% \tiny
% \caption{Evaluation results of our method on 3DMatch dataset.}
% \label{table1}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l|c|c|c|c|c}
% \toprule
% \noalign{\vspace{-0.5ex}}
% \multicolumn{1}{l}{\# Samples} & \multicolumn{1}{c}{5000} & \multicolumn{1}{c}{2500} & \multicolumn{1}{c}{1000} & \multicolumn{1}{c}{500} & \multicolumn{1}{c}{250} \\
% \noalign{\vspace{-0.5ex}}
% \midrule
% \noalign{\vspace{-0.5ex}}
% \multicolumn{6}{c}{\textit{Feature Matching Recall (\%)}$\uparrow$} \\
% \noalign{\vspace{-0.5ex}}
% \midrule
% PerfectMatch~\cite{gojcic2019perfect} & 95.0 & 94.3 & 92.9 & 90.1 & 82.9 \\
% FCGF~\cite{choy2019fully} & 97.4 & 97.3 & 97.0 & 96.7 & 96.6 \\
% D3Feat~\cite{bai2020d3feat} & 95.6 & 94.3 & 95.6 & 94.3 & 91.0 \\
% SpinNet~\cite{ao2021spinnet} & 97.6 & 97.2 & 96.8 & 95.5 & 96.5 \\
% Predator~\cite{huang2021predator} & 96.6 & 96.6 & 96.5 & 96.3 & 95.3 \\
% YOHO~\cite{wang2022you} & \textbf{98.2} & 97.6 & 97.5 & 97.7 & 96.0 \\
% CoFiNet~\cite{yu2021cofinet} & \underline{98.1} & \underline{98.3} & \underline{98.1} & 98.2 & 98.3 \\
% GeoTransformer~\cite{qin2022geometric} & 97.9 & 97.9 & 97.9 & 97.9 & 97.6 \\
% PCR-CG~\cite{zhang2022pcr} & 97.4 & 97.5 & 97.7 & 97.3 & 97.6 \\
% OIF-Net~\cite{yang2022one} & \underline{98.1} & 98.1 & 97.9 & \underline{98.4} & \underline{98.4} \\
% RoITr~\cite{yu2023rotation} & 98.0 & 98.0 & 97.9 & 98.0 & 97.9 \\
% SIRA-PCR~\cite{chen2023sira} & \textbf{98.2} & \textbf{98.4} & \textbf{98.4} & \textbf{98.5} & \textbf{98.5} \\
% IGASA (\textit{ours}) & \textbf{98.2} & 97.8 & 97.8 & 97.9 & 97.8 \\
% \midrule
% \noalign{\vspace{-0.5ex}}
% \multicolumn{6}{c}{\textit{Registration Recall (\%)}$\uparrow$} \\
% \noalign{\vspace{-0.5ex}}
% \midrule
% PerfectMatch~\cite{gojcic2019perfect} & 78.4 & 76.2 & 71.4 & 67.6 & 50.8 \\
% FCGF~\cite{choy2019fully} & 85.1 & 83.4 & 82.7 & 81.6 & 76.6 \\
% D3Feat~\cite{bai2020d3feat} & 81.6 & 84.5 & 83.4 & 82.7 & 77.9 \\
% SpinNet~\cite{ao2021spinnet} & 86.6 & 85.8 & 85.5 & 83.5 & 79.7 \\
% Predator~\cite{huang2021predator} & 89.0 & 89.9 & 90.6 & 88.5 & 86.6 \\
% YOHO~\cite{wang2022you} & 90.8 & 90.3 & 89.1 & 88.6 & 84.5 \\
% CoFiNet~\cite{yu2021cofinet} & 92.0 & 91.8 & 91.8 & 91.4 & 91.2 \\
% GeoTransformer~\cite{qin2022geometric} & 92.0 & 91.8 & 91.1 & 91.4 & 92.0 \\
% PCR-CG~\cite{zhang2022pcr} & 89.4 & 90.7 & 90.0 & 88.7 & 86.8 \\
% OIF-Net~\cite{yang2022one} & 92.4 & 91.9 & 91.8 & 91.4 & 91.0 \\
% RoITr~\cite{yu2023rotation} & 91.9 & 91.7 & 91.8 & 91.4 & 91.0 \\
% SIRA-PCR~\cite{chen2023sira} & \underline{93.6} & \underline{93.9} & \underline{93.9} & \underline{92.7} & \underline{92.4} \\
% IGASA (\textit{ours}) & \textbf{94.6} & \textbf{94.5} & \textbf{94.5} & \textbf{94.4} & \textbf{94.3} \\
% \midrule
% \noalign{\vspace{-0.5ex}}
% \multicolumn{6}{c}{\textit{Inlier Ratio (\%)}$\uparrow$} \\
% \noalign{\vspace{-0.5ex}}
% \midrule
% PerfectMatch~\cite{gojcic2019perfect} & 36.0 & 32.5 & 26.4 & 21.5 & 16.4 \\
% FCGF~\cite{choy2019fully} & 56.8 & 54.1 & 48.7 & 42.5 & 34.1 \\
% D3Feat~\cite{bai2020d3feat} & 39.0 & 38.8 & 40.4 & 41.5 & 41.8 \\
% SpinNet~\cite{ao2021spinnet} & 47.5 & 44.7 & 39.4 & 33.9 & 27.6 \\
% Predator~\cite{huang2021predator} & 58.0 & 58.4 & 57.1 & 54.1 & 49.3 \\
% YOHO~\cite{wang2022you} & 64.4 & 60.7 & 55.7 & 46.4 & 41.2 \\
% CoFiNet~\cite{yu2021cofinet} & 49.8 & 51.2 & 51.9 & 52.2 & 52.2 \\
% GeoTransformer~\cite{qin2022geometric} & 71.9 & 75.2 & 76.0 & 82.2 & 85.1 \\
% OIF-Net~\cite{yang2022one} & 62.3 & 65.2 & 66.8 & 67.1 & 67.5 \\
% RoITr~\cite{yu2023rotation} & \underline{82.6} & \underline{82.8} & 83.0 & 83.0 & 83.0 \\
% SIRA-PCR~\cite{chen2023sira} & 70.8 & 78.3 & \underline{83.7} & \underline{85.9} & \underline{87.4} \\
% IGASA (\textit{ours}) & \textbf{87.9} & \textbf{87.8} & \textbf{87.9} & \textbf{87.9} & \textbf{87.9} \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

% \begin{table}[t]
% \centering
% \tiny
% \caption{Evaluation results of our method on 3DLoMatch dataset}
% \label{table2}
% \resizebox{\columnwidth}{!}{ % Resizing the table to fit the single column width
% \begin{tabular}{l|c|c|c|c|c}
% \toprule % 最上方的加粗线
% \noalign{\vspace{-0.5ex}}
% \multicolumn{1}{l}{\# Samples} & \multicolumn{1}{c}{5000} & \multicolumn{1}{c}{2500} & \multicolumn{1}{c}{1000} & \multicolumn{1}{c}{500} & \multicolumn{1}{c}{250} \\
% \noalign{\vspace{-0.5ex}}
% \midrule
% \noalign{\vspace{-0.5ex}}
% \multicolumn{6}{c}{\textit{Feature Matching Recall (\%) }$\uparrow$} \\
% \noalign{\vspace{-0.5ex}}
% \midrule
% PerfectMatch~\cite{gojcic2019perfect} & 63.6 & 61.7 & 53.6 & 45.2 & 34.2 \\
% FCGF~\cite{choy2019fully} & 76.6 & 75.4 & 74.2 & 71.7 & 67.3 \\
% D3Feat~\cite{bai2020d3feat} & 66.7 & 64.7 & 61.6 & 60.0 & 56.6 \\
% SpinNet~\cite{ao2021spinnet} & 75.3 & 74.9 & 72.5 & 70.0 & 63.6 \\
% Predator~\cite{huang2021predator} & 78.6 & 76.7 & 75.7 & 75.7 & 72.9 \\
% YOHO~\cite{wang2022you} & 79.4 & 78.1 & 76.3 & 73.8 & 69.1 \\
% CoFiNet~\cite{yu2021cofinet} & 83.1 & 83.5 & 83.3 & 83.1 & 82.6 \\
% GeoTransformer~\cite{qin2022geometric} & 88.3 & 88.6 & 88.8 & \underline{88.6} & \underline{88.3} \\
% PCR-CG~\cite{zhang2022pcr} & 80.4 & 82.2 & 82.6 & 83.2 & 82.8 \\
% OIF-Net~\cite{yang2022one} & 84.6 & 85.2 & 85.5 & \underline{88.6} & 87.0 \\
% RoITr~\cite{yu2023rotation} & \textbf{89.6} & \textbf{89.6} & \textbf{89.5} & \textbf{89.4} & \textbf{89.3} \\
% SIRA-PCR~\cite{chen2023sira} & \underline{88.8} & \underline{89.0} & \underline{88.9} & \underline{88.6} & 87.7 \\
% IGASA (\textit{ours}) & 82.1 & 80.5 & 80.5 & 80.5 & 80.4 \\
% \midrule
% \noalign{\vspace{-0.5ex}}
% \multicolumn{6}{c}{\textit{Registration Recall (\%)} $\uparrow$} \\
% \noalign{\vspace{-0.5ex}}
% \midrule
% PerfectMatch~\cite{gojcic2019perfect} & 33.0 & 29.0 & 23.7 & 11.0 & 15.9 \\
% FCGF~\cite{choy2019fully} & 74.4 & 70.4 & 67.2 & 63.4 & 61.4 \\
% D3Feat~\cite{bai2020d3feat} & 69.4 & 60.2 & 58.5 & 51.6 & 42.6 \\
% SpinNet~\cite{ao2021spinnet} & 68.9 & 59.6 & 56.8 & 50.0 & 49.1 \\
% Predator~\cite{huang2021predator} & 61.2 & 61.2 & 62.4 & 60.8 & 58.1 \\
% YOHO~\cite{wang2022you} & 67.5 & 68.0 & 62.2 & 63.4 & 61.9 \\
% CoFiNet~\cite{yu2021cofinet} & 75.0 & \underline{74.8} & 74.2 & 74.1 & 73.5 \\
% GeoTransformer~\cite{qin2022geometric} & \underline{75.5} & \underline{74.8} & 74.6 & \underline{74.6} & \underline{75.3} \\
% PCR-CG~\cite{zhang2022pcr} & 66.3 & 67.2 & 69.0 & 68.5 & 65.0 \\
% OIF-Net~\cite{yang2022one} & 74.7 & \underline{74.8} & \underline{74.8} & 74.2 & 73.6 \\
% RoITr~\cite{yu2023rotation} & 74.7 & \underline{74.8} & \underline{74.8} & 74.2 & 73.6 \\
% SIRA-PCR~\cite{chen2023sira} & 73.5 & 73.9 & 73.0 & 73.4 & 71.1 \\
% IGASA (\textit{ours}) & \textbf{76.5} & \textbf{76.5} & \textbf{76.3} & \textbf{76.4} & \textbf{76.4} \\
% \midrule
% \noalign{\vspace{-0.5ex}}
% \multicolumn{6}{c}{\textit{Inlier Ratio (\%) }$\uparrow$} \\
% \noalign{\vspace{-0.5ex}}
% \midrule
% PerfectMatch~\cite{gojcic2019perfect} & 11.4 & 10.1 & 8.0 & 6.4 & 4.8 \\
% FCGF~\cite{choy2019fully} & 21.4 & 20.0 & 17.2 & 14.8 & 11.6 \\
% D3Feat~\cite{bai2020d3feat} & 13.2 & 13.1 & 14.0 & 14.6 & 15.0 \\
% SpinNet~\cite{ao2021spinnet} & 20.5 & 19.0 & 16.3 & 13.8 & 11.1 \\
% Predator~\cite{huang2021predator} & 26.7 & 28.1 & 28.3 & 27.5 & 25.8 \\
% YOHO~\cite{wang2022you} & 25.9 & 23.3 & 22.6 & 18.2 & 15.0 \\
% CoFiNet~\cite{yu2021cofinet} & 24.4 & 25.9 & 26.7 & 26.8 & 26.9 \\
% GeoTransformer~\cite{qin2022geometric} & 43.5 & 45.3 & 46.2 & 52.9 & 57.7 \\
% OIF-Net~\cite{yang2022one} & 27.5 & 30.0 & 31.2 & 32.6 & 33.1 \\
% RoITr~\cite{yu2023rotation} & \underline{54.3} & \underline{54.6} & 55.1 & 55.2 & 55.3 \\
% SIRA-PCR~\cite{chen2023sira} & 43.3 & 49.0 & \underline{55.9} & \underline{58.8} & \underline{60.7} \\
% IGASA (\textit{ours}) & \textbf{61.6} & \textbf{61.5} & \textbf{61.5} & \textbf{61.6} & \textbf{61.4} \\
% \bottomrule % 底部加粗框线
% \end{tabular}
% }
% \end{table}

\textbf{Dataset.} The 3DMatch~\cite{zeng20173dmatch} and 3DLoMatch~\cite{huang2021predator} datasets are constructed from RGB-D data. The 3DMatch dataset contains 62 indoor scenes, with 46 scenes allocated for training, 8 for validation, and 8 for testing. Each scene in the 3DMatch dataset consists of point cloud pairs with at least a 30\% overlap. In contrast, the point clouds in the 3DLoMatch dataset have a smaller overlap, ranging from 10\% to 30\%.

\textbf{Metrics.} In our evaluation, we employ three key metrics to comprehensively assess registration performance: Inlier Ratio (IR), Feature Matching Recall (FMR), and Registration Recall (RR). The IR quantifies the proportion of candidate correspondences with residual errors below a set threshold ($e.g.,$ 0.1 m) under the ground-truth transformation. FMR measures the fraction of point cloud pairs that achieve an inlier ratio above a designated threshold ($e.g.,$ 5\%).

\textbf{Registration results.} In summary, IGASA outperforms state-of-the-art methods on both datasets, excelling in RR, IR, and FMR. \rev{We compare our method IGASA, with recent methods: %PerfectMatch~\cite{gojcic2019perfect},D3Feat~\cite{bai2020d3feat}, SpinNet~\cite{ao2021spinnet}, 
FCGF~\cite{choy2019fully},  Predator~\cite{huang2021predator}, YOHO~\cite{wang2022you}, CoFiNet~\cite{yu2021cofinet}, GeoTransformer~\cite{qin2022geometric}, PCR-CG~\cite{zhang2022pcr}, OIF-Net~\cite{yang2022one}, RoITr~\cite{yu2023rotation}, FeatSync~\cite{hu2024featsync}, OT-CA~\cite{guo2024learning} and SIRA-PCR~\cite{chen2023sira}. The outcomes for 3DMatch and 3DLoMatch are displayed in \cref{table1}. Our method demonstrates significant improvements in multiple evaluation metrics. For a more comprehensive evaluation, please refer to Table S.IV in the Supplementary Material.}

To 3DMatch dataset, the results indicate that IGASA achieves a competitive FMR; for instance, at 5000 samples, it attains an FMR of 98.2\%, comparable to YOHO~\cite{wang2022you} and SIRA‐PCR~\cite{chen2023sira}. However, under sparser conditions ($e.g.,$ 250 or 500 samples), IGASA’s FMR is slightly lower than some competing methods, suggesting that feature robustness under limited samples may be an area for further improvement.
In terms of RR, IGASA consistently outperforms the compared methods, recording values of 94.6\%, 94.5\%, 94.5\%, 94.4\%, and 94.3\% as the sample size decreases from 5000 to 250.
Additionally, IGASA demonstrates stable performance in the IR metric, maintaining 87.9\% across most sample sizes. This result is notably higher than those of methods such as GeoTransformer~\cite{qin2022geometric}, RoITr~\cite{yu2023rotation}, and SIRA‐PCR~\cite{chen2023sira}, reflecting robust inlier extraction and enhanced noise resistance.

The results in \cref{table1} show that IGASA performs well on the 3DLoMatch dataset across key metrics: FMR, RR and IR. In RR, IGASA performs best among all methods, with a peak of 76.5\% at 5000 and 2500 samples, surpassing competitors like RoITr~\cite{yu2023rotation} and SIRA-PCR~\cite{chen2023sira}. Additionally, in terms of IR, IGASA leads with 61.6\% at 5000 samples and maintains high values across smaller sample sizes, demonstrating superior inlier extraction.
Overall, these results demonstrate IGASA's potential to outperform traditional point cloud registration methods.

\textbf{Qualitative results.} \cref{figurelabe4} provides a series of qualitative registration results on 3DM(Lo)atch, which emphasize the advantages of IGASA in terms of registration results.

\subsection{Outdoor Benchmark: KITTI odometry}

\textbf{Dataset.} KITTI~\cite{geiger2013vision} is a widely recognized benchmark for autonomous driving, consisting of 11 outdoor driving sequences captured by LiDAR sensors. Following common protocols established in prior work, sequences 0-5 are used for training, 6-7 for validation, and 8-10 for testing. 

\begin{table}[t]
\centering
\caption{Registration performance on KITTI dataset.}
\label{table3}
\resizebox{0.8\columnwidth}{!}{ 
\begin{tabular}{lccc}
\toprule
Model & RTE (cm) & RRE (°) & RR (\%) \\
\midrule
3DFeat-Net~\cite{yew20183dfeat}    & 25.9 & 0.25 & 96.0  \\
FCGF~\cite{choy2019fully}           & 9.5  & 0.30 & 96.6  \\
% D3Feat~\cite{bai2020d3feat}         & 7.2  & 0.30 & \underline{99.8}  \\
% SpinNet~\cite{ao2021spinnet}        & 9.9  & 0.47 & 99.1 \\
Predator~\cite{huang2021predator}       & 6.8  & 0.27 & \underline{99.8} \\
CoFiNet~\cite{yu2021cofinet}        & 8.2  & 0.41 & \underline{99.8} \\
HRegNet~\cite{lu2021hregnet}       & 12  & 0.29 & 99.7 \\
GeoTransformer~\cite{qin2022geometric}  & 6.8  & \underline{0.24} & \underline{99.8} \\
OIF-Net~\cite{yang2022one}         & \underline{6.5}  & \textbf{0.23} & \underline{99.8} \\
MAC~\cite{zhang20233d}            & 8.5  & 0.40 & 99.5 \\
IGASA (\textit{ours})           & \textbf{4.6}  & \underline{0.24} & \textbf{100.0} \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table}

\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{fig5.pdf}
  \caption{\rev{Qualitative registration results on the KITTI odometry benchmark. We visualize four representative driving scenes characterized by large spatial extents and varying structural distinctiveness. The first row displays the initial unaligned input pairs (Source: Blue, Target: Yellow), illustrating significant initial pose discrepancies. The second row shows the registration results achieved by IGASA. The red rectangular boxes highlight specific regions with sharp structural boundaries, such as road curbs and intersection corners. Note that despite the limited overlap and noise typical of outdoor LiDAR scans, our method precisely aligns fine-grained structures such as trees, vehicles, and road boundaries.}}
  \label{figurelabe5}
  \vspace{-5mm}
\end{figure*}

\textbf{Metrics.} To evaluate the performance, we adopt three crucial metrics. RR, Relative Rotation Error (RRE), and Relative Translation Error (RTE). RR quantifies the proportion of point cloud pairs for which the estimated transformation meets a predefined accuracy threshold. Meanwhile, RRE measures the angular discrepancy between the estimated and ground-truth rotations, and RTE evaluates the distance between the estimated and true translation vectors.

\textbf{Registration Results.} For the KITTI dataset evaluation, as shown in Table \ref{table3}, outperforms all state-of-the-art methods, \rev{including
%D3Feat~\cite{bai2020d3feat}, SpinNet~\cite{ao2021spinnet}, 
3DFeat-Net~\cite{yew20183dfeat}, FCGF~\cite{choy2019fully}, Predator~\cite{huang2021predator}, CoFiNet~\cite{yu2021cofinet}, HRegNet~\cite{lu2021hregnet}, GeoTransformer~\cite{qin2022geometric}, OIF-Net~\cite{yang2022one} and MAC~\cite{zhang20233d}.} Specifically, IGASA achieves an RTE of 4.6 cm, an RRE of 0.24°, and an RR of 100.0\%, which are all the best results among total compared methods. 

Compared to traditional feature-based methods like 3DFeat-Net~\cite{yew20183dfeat} and FCGF~\cite{choy2019fully}, IGASA shows significant improvements. While 3DFeat-Net~\cite{yew20183dfeat} has an RTE of 25.9 cm and a RR of 96.0\%, IGASA's performance in both accuracy and registration recall is superior, demonstrating the strength of the model in handling complex registration tasks.
IGASA also leads the comparison with transformer-based models like GeoTransformer~\cite{qin2022geometric} and OIF-Net~\cite{yang2022one}, achieving higher RR and lower RTE.

\textbf{Qualitative results.} \rev{To further validate the robustness of IGASA in outdoor environments, we present qualitative visualization results on the KITTI dataset in \cref{figurelabe5}. As shown in the second row, our method achieves precise alignment even in scenes with large initial misalignment and repetitive geometric structures. Highlighted by the red rectangular boxes, the tight overlap between the source (blue) and target (yellow) point clouds demonstrates the high accuracy of our estimated 6-DoF pose, particularly around road curbs and structural corners. This visual alignment confirms the effectiveness of the proposed method in capturing fine geometric details.}

\begin{table}[t]
\centering
\caption{Registration performance on nuScenes dataset.}
\label{table4}
\resizebox{0.85\columnwidth}{!}{ 
\begin{tabular}{lccc}
\toprule
Model & RTE (m) & RRE (°) & RR (\%) \\
\midrule
% Point-to-Point ICP~\cite{besl1992method}    & 0.25 & 0.25 & 18.8  \\
% Point-to-Plane ICP~\cite{besl1992method}           & 0.15  & 0.21 & 36.8  \\
FGR~\cite{zhou2016fast}         & 0.71  & 1.01 & 32.2  \\
% RANSAC~\cite{fischler1981random}        & 0.21  & 0.74 & 60.9 \\
DCP~\cite{wang2019deep}       & 1.09  & 2.07 & 56.8 \\
IDAM~\cite{li2020iterative}        & 0.47  & 0.79 & 88.0 \\
FMR~\cite{huang2020feature}       & 0.60  & 1.61 & 92.1 \\
DGR~\cite{choy2020deep}  & 0.21  & 0.48 & \underline{98.4} \\
HRegNet~\cite{lu2021hregnet}      & \underline{0.18}  & \underline{0.45} & \textbf{99.9} \\
IGASA (\textit{ours})           & \textbf{0.12}  & \textbf{0.21} & \textbf{99.9} \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table}

\subsection{Outdoor Benchmark: nuScenes odometry}
\textbf{Dataset.} NuScenes~\cite{caesar2020nuscenes} is a large-scale dataset designed for autonomous driving, capturing diverse outdoor scenarios with data from a complete suite of sensors. It comprises 850 scenes for training and validation, with an additional 150 scenes reserved for testing. We partition the dataset by assigning the first 700 scenes for training while using the remainder for validation. To optimize the processing of raw data, we apply a voxel grid down-sampling with a resolution of 0.3 m, which effectively reduces point cloud density while preserving essential geometric details. 

\textbf{Metrics.} We adopt RR, RRE and RTE to thoroughly assess registration performance.

\textbf{Registration Results.} For LiDAR benchmark nuScenes, we evaluate our IGASA by comparing with several recent state-of-the-art methods~\cite{lu2021hregnet},~\cite{zhou2016fast},~\cite{wang2019deep},~\cite{li2020iterative,huang2020feature},~\cite{choy2020deep} as shown in Table \ref{table4}. The experimental results demonstrate that IGASA outperforms competing methods in point cloud registration. IGASA achieves an RTE of 0.12 m, an RRE of 0.21° and a RR of 99.9\%, surpassing traditional methods. 

\textbf{Qualitative results.} \rev{\cref{figurelabe6} illustrates the registration performance on the nuScenes dataset, which is characterized by sparse LiDAR points and low overlap. Despite the lack of dense geometric features, IGASA successfully recovers the correct transformation parameters. As highlighted by the red rectangular boxes in the bottom row, the aligned results demonstrate that our HCLA module effectively captures global context from sparse data, ensuring reliable registration even when local features are ambiguous or missing.}

\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{fig6.pdf}
  \caption{\rev{Qualitative registration results on the nuScenes dataset. These scenes exhibit extreme sparsity and non-uniform point density, which pose significant challenges for correspondence estimation. The first row shows the raw, unaligned point clouds. The second row presents the aligned results from IGASA. The red rectangular boxes highlight specific regions containing aligned sparse geometric cues, such as ground scan lines and structural edges. It can be observed that IGASA robustly handles the sparse geometry, effectively aligning the ground plane and sparse vertical structures ($e.g.,$ traffic signs), demonstrating its efficacy in low-texture environments.}}
  \label{figurelabe6}
  \vspace{-5mm}
\end{figure*}

\subsection{Ablation Experiment}



\subsubsection{Related Modules in IGASA}

\rev{To assess the individual contribution of each component, we conducted a comprehensive ablation study on the 3DMatch dataset, as summarized in \cref{table5}. The baseline model, which utilizes a standard UNet-like backbone without the proposed attention and refinement modules, yields a RR of only 89.6\%. The integration of the HCLA module significantly boosts the recall to 92.8\%, a substantial improvement that validates the importance of bridging the semantic gap. This gain indicates that the SGIRA and SAIGA units effectively guide the feature learning process, ensuring that local geometry is semantically aligned before matching.}

\rev{Most notably, the addition of the IGAR module further elevates the performance to 94.6\%. This improvement is particularly evident in the IR, which rises from 79.2\% to 87.9\%. This finding underscores the critical role of the iterative refinement stage. While HCLA provides a robust initial alignment, it is the dynamic geometric consistency weighting within IGAR that effectively suppresses residual outliers and fine-tunes the pose, ensuring high-precision registration even in complex scenes. The complete IGASA framework thus achieves the optimal balance between robust feature extraction and precise geometric alignment.}


% In this section, we perform a series of ablation experiments to evaluate the contributions of three modules in IGASA. The detailed results of these experiments are presented in \cref{table5}.

% We chose to ablate indoor dataset for coarse matching because it is more challenging, evaluating the RR over the entire dataset. We also introduced FMR and IR to assess matching performance.

% In the first experiment, removing the HPA module led to a drop in all metrics. In the second experiment, removing the HCLA module caused a further decrease in RR, from 94.6\% to 92.8\%, highlighting its importance in ensuring feature consistency. The third experiment showed a decrease when the IGAR module was removed, with IR falling from 87.9\% to 83.7\%, emphasizing the module's contribution to fine-grained computation.

% Overall, the full IGASA model outperformed all ablated versions across all evaluation metrics. These results confirm the complementary nature of the modules and validate the overall effectiveness of the model.

\begin{table}[t]
\centering
\caption{\rev{Ablation study of key modules in the IGASA framework on the 3DMatch and 3DLoMatch datasets. The results are reported in percentage (\%). Best performance is highlighted in bold. The baseline denotes the network without HCLA and IGAR.}
}
\resizebox{0.9\columnwidth}{!}{ 
\label{table5}
\begin{tabular}{ccc|ccc|ccc}
\toprule
\multicolumn{3}{c}{Module} & \multicolumn{3}{c}{3DMatch} & \multicolumn{3}{c}{3DLoMatch} \\
HPA & HCLA & IGAR & FMR & IR & RR & FMR & IR & RR \\
\midrule
$\checkmark$ & - & - & 92.7 & 80.2  & 91.3 & 72.8 & 49.7 & 70.8 \\ 
- & $\checkmark$ & - & 94.2 & 83.5  & 91.9 & 75.9 & 55.1 & 72.7 \\ 
- & - & $\checkmark$ & 93.0 & 81.7  & 91.5 & 69.2 & 52.6  & 71.5\\
- & $\checkmark$ & $\checkmark$ & 97.2 & 85.2 & 93.4 & 74.3 & 57.6 & 74.2  \\
$\checkmark$ & - & $\checkmark$ & 95.6 & 81.9 & 92.8 & 71.0 & 51.3 & 72.3  \\
$\checkmark$ & $\checkmark$ & - & 96.9 & 83.7 & 93.2 & 78.9 & 53.8 & 73.5 \\
$\checkmark$ & $\checkmark$ & $\checkmark$  & \textbf{98.2} & \textbf{87.9} & \textbf{94.6} & \textbf{82.1} & \textbf{61.6} & \textbf{76.5}  \\
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}

\subsubsection{SGIRA and SAIGA in HCLA Module}

\rev{We further investigate the internal mechanisms of the HCLA module by analyzing the separate contributions of its two sub-components: SGIRA and SAIGA. The quantitative results are presented in Table \ref{table6}.}

\rev{The results reveal a clear hierarchy in feature enhancement. Activating only the SGIRA module improves the FMR from 95.6\ to 96.2\%. This gain is attributed to the semantic filtering capability of SGIRA, which leverages global context to suppress ambiguous local features. Subsequently, enabling only SAIGA yields a further improvement in IR (84.2\%), suggesting that the intrinsic geometric self-attention successfully reinforces spatial distinctiveness, making the descriptors more robust to viewpoint changes.}

\rev{The peak performance is achieved when both components are active (Row 4), yielding an FMR of 98.2\% and an IR of 87.9\%. This significant boost confirms the synergistic relationship between the two units: SGIRA establishes a semantic consensus to filter noise, while SAIGA refines the local geometric details. Together, they ensure that the generated correspondences are both semantically consistent and geometrically precise.}



% The ablation experiments for the HCLA module on the 3DMatch dataset are presented in Table \ref{table6}, focusing on the contributions of the SGIRA and SAIGA components. Four configurations were tested: both components inactive, only SGIRA active, only SAIGA active, and both components active.

% The results demonstrate a clear performance improvement as components are progressively activated. In the baseline configuration (both components inactive), the FMR is 95.6\%, IR is 81.9\%, and RR is 92.8\%. Enabling only SGIRA increases FMR to 96.2\%, IR to 83.3\%, and RR to 93.2\%. With only SAIGA enabled, the performance further improves, with FMR reaching 96.7\%, IR at 84.2\%, and RR at 93.5\%. The best performance is achieved when both components are active, yielding FMR of 98.2\%, IR of 87.9\%, and RR of 94.6\%.

% These results indicate that the integration of SGIRA and SAIGA significantly enhances the point cloud registration performance, confirming their effectiveness within the HCLA module during point cloud registration.

\begin{table}[t]
\centering
\scriptsize % Adjust the font size for the table
%\renewcommand{\arraystretch}{1.5} % Increase vertical spacing (default is 1.0)
\caption{Ablation experiments of the tow components in HCLA module on 3DMatch dataset. The results are reported in percentage (\%). Best performance is highlighted in bold.}
\resizebox{0.65\columnwidth}{!}{ 
\label{table6}
%\resizebox{\columnwidth}{!}{ % Resize the table to fit the single column width
\begin{tabular}{cc|c|c|c}
\toprule
\multicolumn{2}{c}{Module} & \multicolumn{3}{c}{3DMatch}  \\
SGIRA & SAIGA & FMR & IR & RR  \\
\midrule
- & - & 95.6 & 81.9 & 92.8  \\ 
$\checkmark$ & - & 96.2 & 83.3 & 93.2  \\ 
- & $\checkmark$ & 96.7 & 84.2 & 93.5  \\ 
$\checkmark$ & $\checkmark$ & \textbf{98.2} & \textbf{87.9} & \textbf{94.6}  \\
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}

\subsubsection{Analysis of Loss Functions}
\rev{The optimization of IGASA relies on a composite objective function. To validate the necessity of each constraint, we evaluate the performance using combinations of the matching loss ($\mathcal{L}_{\text{mat}}$), keypoint loss ($\mathcal{L}_{\text{key}}$), and dense registration loss ($\mathcal{L}_{\text{den}}$). The results are summarized in Table \ref{table7}.}

\rev{Using any single loss function results in suboptimal performance, indicating that individual constraints are insufficient for the full registration pipeline. For instance, relying solely on $\mathcal{L}_{\text{den}}$ yields a lower IR (71.5\%), as it lacks explicit supervision for coarse correspondence establishment. The combination of $\mathcal{L}_{\text{mat}}$ and $\mathcal{L}_{\text{den}}$ provides a significant boost, highlighting the importance of simultaneously supervising the coarse matching probability and the fine-grained spatial distance.The best results are obtained when all three loss terms are jointly optimized. The inclusion of $\mathcal{L}_{\text{key}}$ further refines the metric by guiding the network to focus on salient overlapping regions. This multi-task supervision strategy ensures that the network learns robust features (via $\mathcal{L}_{\text{mat}}$), identifies reliable keypoints (via $\mathcal{L}_{\text{key}}$), and achieves precise spatial alignment (via $\mathcal{L}_{\text{den}}$), thereby maximizing registration accuracy.}

% The ablation experiments on the impact of different loss functions for point cloud registration, presented in Table \ref{table7}, evaluate the performance using three loss functions: $\mathcal{L}_{\text{mat}}$, $\mathcal{L}_{\text{key}}$, and $\mathcal{L}_{\text{den}}$, with performance measured in terms of FMR, IR, and RR.

% The results show that the combination of two loss functions leads to further improvements in all metrics. Notably, the best performance is achieved when all three loss functions are used together, resulting in significant gains in FMR, IR, and RR.


% These findings indicate that incorporating multiple loss functions enhances the registration accuracy, with the combination of all three providing the most substantial improvement.

\begin{table}[t]
\centering
\caption{\rev{Impact of different loss function combinations on registration performance. $\mathcal{L}_{\text{mat}}$, $\mathcal{L}_{\text{key}}$, and $\mathcal{L}_{\text{den}}$ denote the matching, keypoint, and dense registration losses, respectively. The results are reported in percentage (\%). Best performance is highlighted in bold.}}
\label{table7}
%\resizebox{0.8\columnwidth}{!}{ 
\begin{tabular}{cccccc}
\toprule
$\mathcal{L}_{\text{mat}}$&$\mathcal{L}_{\text{key}}$&$\mathcal{L}_{\text{den}}$ & FMR & IR & RR  \\ 
\midrule
$\checkmark$ & - & - & 93.4 & 74.9 & 91.5  \\ 
- & $\checkmark$ & - & 92.8 & 72.2 & 90.3  \\ 
- & - & $\checkmark$ & 93.0 & 71.5 & 90.7  \\
- & $\checkmark$ & $\checkmark$ & 95.8 & 72.5 & 91.3  \\
$\checkmark$ & - & $\checkmark$ & 96.4 & 75.6 & 92.4  \\
$\checkmark$ & $\checkmark$ & - & 96.3 & 77.1 & 92.1  \\
$\checkmark$ & $\checkmark$ & $\checkmark$  & \textbf{98.2} & \textbf{87.9} & \textbf{94.6}  \\
\bottomrule
\end{tabular}
%}
\vspace{-5mm}
\end{table}

\begin{table}[t]
\centering
\caption{\rev{Computational efficiency comparison on the 3DMatch benchmark. Times are measured in seconds (s). The total time represents the sum of feature extraction (Model time) and transformation estimation (Pose time).}}
\label{table8}
%\resizebox{0.8\columnwidth}{!}{ 
\begin{tabular}{lccc}
\toprule
Methods & Model time & Pose time & Total time \\
\midrule
FCGF~\cite{choy2019fully}            & 0.073           & 4.332          & 4.405          \\
D3Feat~\cite{bai2020d3feat}          & 0.035           & 4.472          & 4.506          \\
SpinNet~\cite{ao2021spinnet}         & 84.569          & 3.583          & 88.152         \\
Predator~\cite{huang2021predator}        & \textbf{0.050}  & 7.014          & 7.064          \\
CoFiNet~\cite{yu2021cofinet}         & 0.167           & \textbf{2.493} & \textbf{2.660} \\
GeoTransformer~\cite{qin2022geometric}  & 0.124           & 2.557          & 2.701          \\
HECPG~\cite{xie2024hecpg}        & 0.112           & 2.584          & 2.696          \\
IGASA(\textit{ours}) &0.135&2.628&2.763 \\
\bottomrule
\end{tabular}
%}
\vspace{-5mm}
\end{table}


\subsubsection{\rev{Efficiency Analysis}}

% The~\cref{table8} comprehensively compares the inference times of various point cloud registration methods. It specifically includes model time for feature extraction, pose time for transformation estimation, and total time. SpinNet~\cite{ao2021spinnet} has the highest model time of 84.152 s, while Predator~\cite{huang2021predator} achieves the lowest model time of 0.050 s but has a relatively high pose time of 7.014 s. Our method, IGASA, shows a competitive performance compared to GeoTransformer~\cite{qin2022geometric} and CoFiNet~\cite{yu2021cofinet} with a model time of 0.135 s, pose time of 2.628 s, and a total time of 2.763 s, offering an efficient solution for point cloud registration.

\rev{To evaluate the practical applicability of the proposed framework, we conducted a runtime analysis on the 3DMatch benchmark, comparing IGASA against key baselines and recent state-of-the-art methods~\cite{huang2021predator,ao2021spinnet,qin2022geometric,yu2021cofinet}. The results, summarized in Table \ref{table8}, decompose the total inference time into feature extraction (Model time) and transformation estimation (Pose time).}

\rev{The comparison reveals that classical methods often suffer from extreme computational bottlenecks; for instance, SpinNet requires over 88 seconds per frame due to its voxelization process, and Predator, while fast in feature extraction, incurs a high pose estimation cost (7.014 s) due to its reliance on heavy RANSAC iterations. In contrast, IGASA demonstrates high efficiency with a total inference time of 2.763 s. This performance is highly competitive with leading transformer-based methods such as GeoTransformer (2.701 s) and CoFiNet (2.660 s), and is comparable to the HECPG (2.696 s).}

\rev{Although IGASA incurs a marginal computational overhead of approximately 0.1 s compared to CoFiNet, this increase is attributable to the additional computations required by the dual-unit HCLA module and the iterative refinement in IGAR. Given the significant gains in registration recall and inlier ratio demonstrated in previous sections, this slight increase in latency is a justifiable trade-off. The results confirm that IGASA effectively balances model complexity and execution speed, making it suitable for applications requiring both high precision and reasonable time efficiency.}

==> sec/5_conclusion.tex <==
\section{Conclusion}

% This paper presented IGASA-PCR, an integrated framework that combines geometry-aware refinement and skip-attention modules within a Hierarchical Pyramid Architecture for robust point cloud registration. The Hierarchical Cross-Layer Attention module effectively aligns multi-scale features, enhancing both global semantics and local geometric consistency. The Iterative Geometry-Aware Refinement module further refines point cloud matches using geometric cues, improving accuracy in challenging conditions. Extensive evaluations on the 3D(Lo)Match, KITTI and nuScenes datasets demonstrate that our method outperforms state-of-the-art methods, achieving superior registration accuracy and robustness. The results highlight the efficacy of our multi-resolution feature fusion and iterative refinement strategy. In the future, we aim to optimize the framework for real-time performance and enhance its adaptability to diverse environments, including dynamic and sparse point clouds.

\rev{In this paper, we presented IGASA as an integrated framework for robust point cloud registration through the synergy of geometry-aware refinement and skip-attention mechanisms. The proposed Hierarchical Pyramid Architecture (HPA) provides a structured foundation for multi-scale feature extraction. Within this architecture, the Hierarchical Cross-Layer Attention (HCLA) module effectively bridges the semantic gap by aligning multi-resolution features and enhancing both global semantics and local geometric consistency. Furthermore, the Iterative Geometry-Aware Refinement (IGAR) module improves registration precision by leveraging spatial geometric cues to dynamically suppress outliers through an alternating optimization strategy.}
Extensive evaluations conducted on the 3D(Lo)Match, KITTI, and nuScenes datasets demonstrate that our method consistently outperforms state-of-the-art techniques in terms of accuracy and robustness. These results highlight the efficacy of combining multi-resolution feature fusion with iterative geometric refinement for complex 3D vision tasks. \rev{However, the framework exhibits a slight increase in computational latency due to the iterative nature of the refinement process.}
In the future, we aim to further optimize the framework to enhance its adaptability to highly dynamic environments and explore more efficient architectures for real-time large-scale point cloud processing.

% \section*{Acknowledgements}
% This work was supported in part by NSFC under grant No. 62125305, the Natural Science Basis Research Plan in Shaanxi Province of China under Grant No. 2025JC-JCQN-091 and the Technology Innovation Leading Program of Shaanxi (Program No. 2024QY-SZX-23).
